Attack Resilient Interconnected Second Order Systems: A Game-Theoretic Approach

This paper studies the resilience of second-order networked dynamical systems to strategic attacks. We discuss two widely used control laws, which have applications in power networks and formation control of autonomous agents. In the first control law, each agent receives pure velocity feedback from its neighbor. In the second control law, each agent receives its velocity relative to its neighbors. The attacker selects a subset of nodes in which to inject a signal, and its objective is to maximize the $\mathcal{H}_2$ norm of the system from the attack signal to the output. The defender improves the resilience of the system by adding self-feedback loops to certain nodes of the network with the objective of minimizing the system's $\mathcal{H}_2$ norm. Their decisions comprise a strategic game. Graph-theoretic necessary and sufficient conditions for the existence of Nash equilibria are presented. In the case of no Nash equilibrium, a Stackelberg game is discussed, and the optimal solution when the defender acts as the leader is characterized. For the case of a single attacked node and a single defense node, it is shown that the optimal location of the defense node for each of the control laws is determined by a specific network centrality measure. The extension of the game to the case of multiple attacked and defense nodes is also addressed.

==> CDC2019 (3)/defs.tex <==













\section{Graph Theory}
\label{sec:not}
We use $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ to denote an undirected graph where $\mathcal{V}$ is the set of vertices (or nodes) and   $\mathcal{E}\subseteq \{\{v_i,v_j\}|v_i,v_j\in \mathcal{V}, i\neq j \}$ is the set of undirected edges, where  $e=\{v_i,v_j\}\in \mathcal{E}$ if an only if there exists an undirected edge between $v_i$ and $v_j$.  Let $n=|\mathcal{V}|$. The adjacency matrix of $\mathcal{G}$ is denoted  $A$, where $A_{ij}=1$ if  there is an edge between $v_j$ and $v_i$ in $\mathcal{G}$ and zero otherwise. The {\it neighbors} of vertex $v_i \in \mathcal{V}$ in the graph $\mathcal{G}$ are denoted by the  set $\mathcal{N}_i = \{v_j \in \mathcal{V}~|~\{v_j, v_i\} \in \mathcal{E}\}$. We define the degree  for node $v_i$ as $d_i=\sum_{v_j\in \mathcal{N}_i} A_{ij}$.  The Laplacian matrix of an undirected  graph is denoted by $L = D - A$, where $D = \diag (d_1, d_2, ..., d_n)$. We use $\mathbf{e}_i$ to indicate the $i$-th vector of the canonical basis. The eccentricity $\epsilon (v)$ of a vertex $v$ in a connected graph $\mathcal{G}$ is the maximum graph distance  between $v$ and any other vertex $u \in \mathcal{G}$. The center of a graph is a set of vertices with minimum  eccentricity.   The {\it effective resistance} between a pair of nodes $i$ and $j$, denoted  $R_{ij}$, is the electrical resistance measured across nodes  $i$ and $j$ when the network represents an electrical circuit where each edge $e$ has electrical conductance  $w_e$ \cite{Ghosh2008}. The effective eccentricity $\epsilon_f (v)$ of a vertex $v$ in a connected graph $\mathcal{G}$ is the maximum graph effective resistance between $v$ and any other vertex $u$ of $\mathcal{G}$. The {\it effective center} of a graph is a set of vertices with minimum effective eccentricity.  A degree central node in the network is the node with the largest degree.




\section{System Model and Preliminaries}



\iffalse
\subsection{Notations and Definitions}
\label{sec:not}
We use $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ to denote an undirected graph where $\mathcal{V}$ is the set of vertices (or nodes) and $\mathcal{E}$ is the set of undirected edges where  $\{v_i,v_j\}\in \mathcal{E}$ if an only if there exists an undirected edge between $v_i$ and $v_j$.  Let $|\mathcal{V}|=n$ and define the adjacency matrix for $\mathcal{G}$, denoted by $A_{n\times n}$, to be a matrix  where  $A_{ij}=w_{ij}$ if and only if there is an edge with weight $w_{ij}$ between $v_j$ and $v_i$ in $\mathcal{G}$ (the adjacency matrix will be a symmetric matrix when the graph is undirected). The {\it neighbors} of vertex $v_i \in \mathcal{V}$ in the graph $\mathcal{G}$ are denoted by the set $\mathcal{N}_i = \{v_j \in \mathcal{V}~|~(v_j, v_i) \in \mathcal{E}\}$. We define the degree  for node $v_i$ as $d_i=\sum_{v_j\in \mathcal{N}_i} A_{ij}$.  The Laplacian matrix of an undirected  graph is denoted by $L = D - A$, where $D = \diag (d_1, d_2, ..., d_n)$. We use $\mathbf{e}_i$ to indicate the $i$-th vector of the canonical basis. The eccentricity $\epsilon (v)$ of a vertex $v$ in a connected  graph $\mathcal{G}$ is the maximum graph distance  between $v$ and any other vertex $u$ of $\mathcal{G}$. The center of a graph is a set of vertices with minimum  eccentricity.  The $f$-eccentricity, $\epsilon_f (v)$, of a vertex $v$ in a connected  graph $\mathcal{G}$ is the maximum sum of graph distances  between $v$ and any combination of $f$ vertices $u_1, u_2, ..., u_f$ in $\mathcal{G}$. The $f$-center of a graph is a set of vertices with minimum  $f$-eccentricity.  The {\it effective resistance}, $R_{ij}$, between two vertices $v_i$ and $v_j$ in a graph is the equivalent resistance between these two vertices when we treat the resistance of each edge $e$ as $\frac{1}{w_e}$, where $w_e$ is its weight.











 Consider a power transmission network with $n$ buses $\mathcal{V}=\{1,\ldots,n\}$ and a set of transmission lines $\mathcal{E}$. Here we assume a Kron-reduced transmission network model, where all buses are modeled as generators and branch resistances are neglected \cite{Tegling}. At each bus $i \in \mathcal{V}$, there is a generator with inertia constant $M_i > 0$, damping/droop constant $D_i > 0$, and voltage phase angle $\theta_i$. The dynamics of the $i$th generator is described by the \emph{swing equation}
\begin{equation}
M_i\ddot{\theta}_i+D_i\dot{\theta}_i=P_{m,i}-P_{e,i}+w_i(t),
\label{eqn:mainpower}
\end{equation}
where $P_{m,i}$ is the constant mechanical power input from turbine and $\zeta_i(t)$ models the attack signal applied by an attacker to generator $i$.  The term $P_{e,i}$ is the real electrical power injected from $i$-th generator to the network, given by
\begin{align}
P_{e,i}= \sum_{j\in \mathcal{N}_i}\nolimits V_iV_jB_{ij}\sin(\theta_i-\theta_j),
\label{eqn:gednn}
\end{align}
where $V_i$ is the nodal voltage magnitude and $-B_{ij} < 0$ is the susceptance associated with edge $\{i,j\}\in\mathcal{E}$. We further approximate \eqref{eqn:gednn} using the so-called DC Power Flow, where $V_i \simeq V_j \simeq 1$ and $|\theta_i-\theta_j| <\!\!< 1$, leading to the linear model
$P_{e,i}\approx \sum_{j\in \mathcal{N}_i}\nolimits B_{ij} (\theta_i-\theta_j)$. Substituting this into  \eqref{eqn:mainpower} yields
\begin{align}
M_i\ddot{\theta}_i+D_i\dot{\theta}_i\approx - \sum_{j\in \mathcal{N}_i}\nolimits &B_{ij} (\theta_i-\theta_j)\nonumber\\
&+P_{m,i}+w_i(t)+\zeta_i (t).
\label{eqn:genn}
\end{align}

In this paper we assume homogeneous inertia and damping parameters, i.e., $M_i=M$ and $D_i=D$ for all $i=1,\ldots,n$ similarly to \cite{EmmaTegling}. In order to defend against the attacker's actions, a defender chooses some generators and apply the following feedback law
\begin{align}
u_i(t)=k(\dot{\theta}_{\rm ref}-\dot{\theta}_i(t)),
\label{eqn:genn}
\end{align}
where $\dot{\theta}_{\rm ref}$ is the reference frequency. The objective of the attacker is to inject the attack signal $\zeta_i$ to a set of nodes (generators) in order to deviate the frequency from $\dot{\theta}_{\rm ref}$ as much as possible. On the other hand, the defender chooses some nodes to make a  feedback in order to minimize this deviation. After shifting the equilibrium point of \eqref{eqn:genn} to the origin, the term proportional to $P_{m,i}$ may be removed and the dynamics of the generators can be written in state-space form for $\boldsymbol{\theta}=[\theta_1 , ..., \theta_n]^{\sf T}$ and $\mathbf{w}=[w_1 , ..., w_n]^{\sf T}$ as
\begin{align}
\begin{bmatrix}
       \dot{\boldsymbol{\theta}} \\[0.3em]
     \ddot{\boldsymbol{\theta}}
     \end{bmatrix}=\underbrace{\begin{bmatrix}
       \mathbf{0}_{n} & I_{n}         \\[0.3em]
     -\frac{1}{M}L & -\frac{D}{M}H
     \end{bmatrix}}_{A}\underbrace{\begin{bmatrix}
       {\boldsymbol{\theta}} \\[0.3em]
     \dot{\boldsymbol{\theta}}
     \end{bmatrix}}_{\boldsymbol{\Theta}}
     &+\underbrace{\begin{bmatrix}
       \mathbf{0}     \\[0.3em]
    \frac{1}{M}I_n
     \end{bmatrix}}_{B}\boldsymbol w(t)\nonumber\\
     &+\underbrace{\begin{bmatrix}
       F  & 0     \\[0.3em]
    0& F 
     \end{bmatrix}}_{B}\begin{bmatrix}
       \boldsymbol \zeta_1(t) \\[0.3em]
      \boldsymbol \zeta_2(t)
     \end{bmatrix},
     \label{eqn:powernetwork}
\end{align}
where $L$ is the Laplacian matrix with weights $B_{ij}$,   $H = I_n+ kD_y$ where  $D_y=\diag(\boldsymbol y)$ in which $\boldsymbol y$  is a binary vector, i.e.,  $y_i\in \{0,1\}$, whose $i$-th element is one if node $i$ has a self feedback and it is zero if it does not have a self-feedback loop. Matrix $F$ determines the decisions of the attacker which consists of $F$ (attacks on generators frequencies) and $F$ (attacks on generators dynamics). The set of nodes under attack and the set of nodes with feedback are denoted by $\mathfrak{F}$ and $\mathfrak{D}$, respectively. The performance metric used for this dynamics is the generators frequencies, i.e., $\mathbf{y}= [\mathbf{0} \quad I_n]\boldsymbol{\Theta}=\dot{\boldsymbol \theta}$. 


\fi


Consider a network of  agents $\mathcal{V}$ where each agent follows second-order dynamics
\begin{align}
\dot{x}_i(t)&=v_i(t),\nonumber\\
\dot{v}_i(t)&=u_i(t)+w_i(t),
\label{eqn:111}
\end{align}
where $x_i(t)$ and $v_i(t)$ represent position (or phase) and velocity (or frequency), respectively.  $u_i(t)$ and $w_i(t)$ are the control input and additive disturbance to the dynamics. The control policy can be either of the following two 
 \begin{subequations}
\begin{align}
 u_i&=-\sum_{j\in \mathcal{N}_i}a_{ij}(x_i-x_j)-(b_i+b_0)v_i.\label{subeq2}
\\
u_i&=-\sum_{j\in \mathcal{N}_i}a_{ij}(x_i-x_j)-\sum_{j\in \mathcal{N}_i}b_{ij}(v_i-v_j)-a_0x_i-b_0v_i.
\label{subeq1}
%\label{eqn:laww}
\end{align}
\end{subequations}
Here $a_{ij}, b_{ij}, a_0$ and $b_0$ are nonnegative control gains. 
Control law \eqref{subeq2} uses the {\it relative position} and {\it absolute velocity} as feedbacks whereas \eqref{subeq1} uses both relative position and velocity as control feedbacks. To simplify our analysis, we assume that  $a_{ij}=b_{ij}=1$  and $a_0=b_0=k>0$, where $k$ is called the defender's control gain.\footnote{This parameter is private and only known by the system designer.}  Note that all of the analysis in this paper can be readily extended to the weighted case. Control laws \eqref{subeq2} and \eqref{subeq1} are canonical forms of well-known second-order systems. In particular, \eqref{subeq2} is the linearized swing equation for a network of power generators \cite{swing, PiraniJohnCDC}, and  \eqref{subeq1} describes the formation control of autonomous agents, e.g., a platoon of connected vehicles \cite{atkins}. 


\subsection{Attack Model}
 Let $\mathfrak{F}$ denote the set of nodes under attack. The state of a node which is under attack evolves as 
\begin{align}
\dot{x}_i(t)&=v_i(t)+\zeta_{1i}(t),\nonumber\\
\dot{v}_i(t)&=u_i(t)+w_i(t)+\zeta_{2i}(t), \quad i \in \mathfrak{F},
\label{eqn:aodvjn}
\end{align}
where $\zeta_{1i}(t)$ and $\zeta_{2i}(t)$ are the effects of attack signals on the first and the second states, respectively. In vector form, \eqref{eqn:aodvjn} is given by
\begin{align}
\dot{\boldsymbol{X}}={A}\boldsymbol{X}
     +{B}_1\boldsymbol w(t)
     +{B}_2\boldsymbol \zeta(t),
     \label{eqn:powernetwork}
\end{align}
where $\boldsymbol{X}=[\boldsymbol x \quad \dot{\boldsymbol x}]^T$, $\boldsymbol{\zeta}=[\boldsymbol \zeta_1 \quad {\boldsymbol \zeta_2}]^T$. Depending on whether control law \eqref{subeq2} or \eqref{subeq1} is in place, the matrix $A$ respectively takes on the form
\begin{equation}
A=\begin{bmatrix}
       \mathbf{0}_{n} & I_{n}         \\[0.3em]
     -{L} & -H
     \end{bmatrix}, \hspace{0.6 mm} {\rm or} \hspace{1 mm} A=\begin{bmatrix}
       \mathbf{0}_{n} & I_{n}         \\[0.3em]
  -\bar{L} & -\bar{L}
     \end{bmatrix}, 
     \label{eqn:dy}
\end{equation}
where $\bar{L}\triangleq L+kD_y$ and $H\triangleq I_n+kD_y$ where $D_y=\diag(\boldsymbol y)$. $\boldsymbol y$  is a binary vector, i.e.,  $y_i\in \{0,1\}$, whose $i$-th element is one if node $i$ has a self feedback and zero if it does not. We assume that $D_y$ has at least one nonzero diagonal element so that $\bar{L}$ is non-singular \cite{ArxiveRobutness}. Here  $B_1=[\mathbf{0} \quad I_n]^T$ and $B_2=I_2\otimes F$, since we assume that if node $i$ is under attack, then its both states are affected by the attack signal.
Matrix $B_2$ encodes the decisions of the attacker. The $i$-th row of $F$ has a single 1 if node $i$ is affected by the attack, and all zeros otherwise.  
The set of nodes under attack and the set of nodes with feedback (defense nodes) are denoted by $\mathfrak{F}$ and $\mathfrak{D}$, respectively. An example of attacker and defender actions on a networked system is schematically shown in Fig.~\ref{fig:s1} (a).





\subsection{Attacker-Defender Game}
 Because we do not have a priori knowledge of the frequency contents of the attack signal, we must choose a system norm which captures the average impact of all frequencies of the attack input. We therefore choose system $\mathcal{H}_2$ norm, which is widely used to measure the level of coherence in synchronization of coupled oscillators \cite{Bamieh2, Tegling}. We first calculate the $\mathcal{H}_2$ norm of \eqref{eqn:powernetwork}. 

\begin{proposition}\label{prop:h2normsdouble}
The $\mathcal{H}_2$ norms of \eqref{eqn:powernetwork}  from the attack signal $\boldsymbol{\zeta}(t)$ to output $\boldsymbol y=\dot{\boldsymbol x}$  for control laws \eqref{subeq2} and \eqref{subeq1} are
\begin{align}
||G_1||^2_2&=\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1}d_i+
\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1},\nonumber\\
||G_2||^2_2&=\frac{1}{2}f+
\frac{1}{2}\sum_{i\in \mathfrak{F}}\bar{L}_{ii}^{-1},
\label{eqn:biaubv}
\end{align}
 where $f$ is the number of attacked nodes, $G_1$ and $G_2$ are transfer functions of  \eqref{eqn:powernetwork} from $\boldsymbol{\zeta}(t)$ to  $\dot{\boldsymbol x}$  for control laws \eqref{subeq2} and \eqref{subeq1}, respectively. $H_{ii}^{-1}$ and $\bar{L}_{ii}^{-1}$ are the $i$-th diagonal elements of $H^{-1}$ and $\bar{L}^{-1}$, respectively.
\end{proposition}
Now, we formally define the attacker-defender game.
\begin{definition}[\textbf{Attacker-Defender Game}]
The attacker chooses a set of $f$ nodes to attack, $\mathfrak{F}\subseteq \mathcal{V}$, in order to maximize the  $\mathcal{H}_2$ norm from the attack signal $\boldsymbol \zeta (t)$ to the output $\boldsymbol y=\dot{\boldsymbol x}$. The defender places local feedback control at $f$ nodes, $\mathfrak{D}\subseteq \mathcal{V}$, to minimize the system $\mathcal{H}_2$ norm.\footnote{Due to the lack of knowledge of the number of attack signals,  the defender considers $f$ as an upper bound of the number of attacked nodes and acts based on this worst-case scenario.} The result is a zero-sum game in which the payoff, based on \eqref{eqn:biaubv}, is given by
\begin{align}\label{eqn:objectives}
J_1(\mathfrak{F}, \mathfrak{D})&=\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1}d_i
+
\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1},\nonumber\\
J_2(\mathfrak{F}, \mathfrak{D})&=\frac{1}{2}f+
\frac{1}{2}\sum_{i\in \mathfrak{F}}\bar{L}_{ii}^{-1}.
\end{align}
The set of attacked nodes $\mathfrak{F}$ determine matrix $B_2$,  and the set of defense nodes   $\mathfrak{D}$ determines matrix $D_y$  and consequently matrices $H$ and $\bar{L}$  in \eqref{eqn:dy}.
\end{definition}
\iffalse
\begin{tcolorbox}
\textbf{Attacker-Defender Game:} The attacker chooses a set of $f$ nodes to attack, $\mathfrak{F}\subseteq \mathcal{V}$, in order to maximize the  $\mathcal{H}_2$ norm from the attack signal $\boldsymbol \zeta (t)$ to the output $\boldsymbol y=\dot{\boldsymbol x}$. The defender places local feedback control at $f$ nodes, $\mathfrak{D}\subseteq \mathcal{V}$, to minimize the system $\mathcal{H}_2$ norm.\footnote{Due to the lack of knowledge of the number of attack signals,  the defender considers $f$ as an upper bound of the number of attacked nodes and acts based on this worst-case scenario.} The result is a zero-sum game in which the payoff, based on \eqref{eqn:biaubv}, is given by
\begin{align}\label{eqn:objectives}
J_1(\mathfrak{F}, \mathfrak{D})&=\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1}d_i
+
\frac{1}{2}\sum_{i\in \mathfrak{F}}H_{ii}^{-1},\nonumber\\
J_2(\mathfrak{F}, \mathfrak{D})&=\frac{1}{2}f+
\frac{1}{2}\sum_{i\in \mathfrak{F}}\bar{L}_{ii}^{-1}.
\end{align}
The set of attacked nodes $\mathfrak{F}$ determine matrix $B_2$,  and the set of defense nodes   $\mathfrak{D}$ determines matrix $D_y$  and consequently matrices $H$ and $\bar{L}$  in \eqref{eqn:dy}.
\end{tcolorbox}
\fi

The actions of the attacker and the defender, when $f$ nodes are under attack and ${f}$ nodes are defended,  define a matrix game $\mathcal{M}_{\binom{n}{{f}}\times \binom{n}{{f}}}$. Here $\mathcal{M}_{ij}=J(\mathfrak{F}_j,\mathfrak{D}_i)$, where $\mathfrak{F}_j$ corresponds to the set chosen by the attacker and $\mathfrak{D}_i$ corresponds to the set chosen by the defender. In other words, the attacker,  the maximizer, chooses columns of matrix $\mathcal{M}$ and the defender, the minimizer, chooses the rows.


\begin{figure}[t!]
\centering
\includegraphics[scale=.35]{statement.pdf}
\caption{(a) An example of an attacker-defender game and matrices $H$ and $\bar{L}$, (b) graph topology discussed in example \ref{exp:alfdkf}, (c) a graph structure where $\Delta_1=\Delta_2$, thus does not admit NE, (d) star graph admits largest threshold for $k$ over all connected graphs as $\Delta_1=n-1$ and $\Delta_2=1$. }
\label{fig:s1}
\end{figure}
























\section{Attacker-Defender Game on $J_1(\mathfrak{F}, \mathfrak{D})$}

In this section, we discuss  equilibrium strategies for the attacker-defender game when the control law is \eqref{subeq2}. First, consider a single attacked node and single defense node. 

\subsection{Single Attacked-Single defense Nodes}

In this case, attacker's payoff is 
\begin{align}\label{eqn:objectsives}
J(\mathfrak{F}, \mathfrak{D})=\frac{H_{ii}^{-1}}{2}\left( d_i+1 \right), \quad i\in \mathfrak{F}.
\end{align}
A Nash equilibrium may not exist, as discussed in the following example. 
\begin{example}
For the path graph of length 3 shown in Fig.~\ref{fig:s1} (b), payoff matrix becomes
\begin{align}
\mathcal{M}=\frac{1}{2}\begin{bmatrix}
      \frac{2}{k+1} & 3 & 2        \\[0.3em]
     2 &  \frac{3}{k+1} & 2 \\[0.3em]
     2 & 3 & \frac{2}{k+1}
     \end{bmatrix},
     \label{eqn:graminnn}
\end{align}
where the attacker (maximizer) chooses columns and the defender (minimizer) chooses the rows. For $k\leq \frac{1}{2}$ both the attacker and defender choose node 2 at NE, and the equilibrium payoff is
 $J^*=\frac{3}{2k+2}$. For $k$ bigger than this threshold, there is no NE for the game.
\label{exp:alfdkf}
\end{example}

The following is a necessary and sufficient condition for the existence of an NE for the attacker-defender game. 
\begin{proposition}\label{prop:necsufgame1}

Suppose that in the game on $J_1(\mathfrak{F}, \mathfrak{D})$ in  \eqref{eqn:objectives}, there are one attacked and one defense nodes.
Then there exists an NE if and only if $k\leq \frac{\Delta_1-\Delta_2}{\Delta_2+1}$, where $\Delta_1$ and $\Delta_2$ are the largest and second largest degrees of nodes in graph $\mathcal{G}$. In this case, the game value is $J^*=\frac{\Delta_1+1}{2k+2}$ and the NE strategy is that both attacker and defender choose the node(s) with the largest degree.
\end{proposition}

\begin{remark}
According to Proposition \ref{prop:necsufgame1}, the value of $k$ which ensures the existence of NE is limited by the gap between the largest and the second largest degrees in the network. For the cases where this does not hold, e.g., when the node with the largest degree is not unique as in Fig.~\ref{fig:s1} (c), there is no NE. Moreover,  the largest possible threshold for graphs on $n$ vertices corresponds to the star graph in which the threshold becomes $\frac{n-2}{2}$, as in Fig.~\ref{fig:s1} (d).
\end{remark}

When there is no NE, we instead analyze a Stackelberg game in which the defender acts as the leader. We can write $J_1(\mathfrak{F},\mathfrak{D})$ in \eqref{eqn:objectives} as
 $$J_1(\mathfrak{F},\mathfrak{D})=\frac{1}{2}\trace \left(F^T({L}+I)H^{-1}F \right).$$
As leader, the defender solves the following optimization problem
 \begin{equation}\label{eqn:stackd}
J^*(D_y)=\min_{D_y}\frac{1}{2}\trace \left(F^{*^T}(D_y)({L}+I)H^{-1}F^{*^T}(D_y) \right)
\end{equation}
where $D_y$ is chosen over all $f$ defense nodes in $\mathcal{V}$. $F^*(D_y)$ is the best response of the attacker when the strategy of the defender is $D_y$, i.e., $F^*(D_y)$ is the solution of the following optimization problem
 \begin{equation}\label{eqn:stack}
F^*(D_y)=\arg\max_F\frac{1}{2}\trace \left(F^T({L}+I)H^{-1}F \right),
\end{equation}
where $F$ is chosen over all ${f}$ attacked nodes in $\mathcal{V}$.
 Unlike NE,  a Stackelberg game always admits an equilibrium strategy.
 \begin{remark}
We  note that for the attacker to play the Stackelberg game, i.e., find the optimal strategy \eqref{eqn:stack}, it is not  necessary to know the exact value of the feedback gain $k$. According to proposition \ref{prop:necsufgame1} and Theorem \ref{thm:multistack}, which comes later, it is sufficient for the attacker to only know if $k$ is above or below the threshold $\frac{\Delta_1-\Delta_2}{\Delta_2+1}$ in order to find its best response strategy.
\end{remark}

The following theorem,  characterizes the equilibrium of the Stackelberg game.

\begin{theorem}\label{thm:necsuefgame}
Consider a Stackelberg attacker-defender game on $J_1(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives}  in which there exists a single attacked node and single defense node, the defender as the game leader, and $k> \frac{\Delta_1-\Delta_2}{\Delta_2+1}$.  Then the equilibrium strategy corresponds to the case where the defender chooses $v=\arg\max_{i\in \mathcal{V}}d_i$, i.e., the node with the largest degree. In this case, the attacker's best response will be $\bar{v}=\arg\max_{i\in \mathcal{V}\setminus v}d_i$, i.e., the node with the second largest degree.
\end{theorem}

The following example discusses the role of the threshold $\bar{k}=\frac{\Delta_1-\Delta_2}{\Delta_2+1}$ in the attacker's strategy.

\begin{example}
For the graph shown in Fig.~\ref{fig:s2} we have $\Delta_1=3, \Delta_2=2$. Hence, the threshold is $\bar{k}=\frac{1}{3}$. The attacker's decisions are plotted with respect to the defender's best action, i.e., the node with the largest degree. For $k=0.1<\bar{k}$, the attacker's best action is the node with the largest degree (as follows from Proposition \ref{prop:necsufgame1}) and for $k=1>\bar{k}$, the attacker's best response is the node with the second largest degree (as follows from Theorem  \ref{thm:necsuefgame}). For $k=\bar{k}$, the payoff will be the same when the attacker chooses either nodes 3 or 4.
\end{example}


\begin{figure}[t!]
\centering
\includegraphics[scale=.35]{strategy.pdf}
\caption{The effect of the feedback value $k$ on attacker's best response. The defender has chosen node 3 (its optimal decision). }
\label{fig:s2}
\end{figure}
\iffalse
\begin{remark}
According to Theorem \ref{thm:necsuefgame}, as the optimal game value is $J^*=\frac{\Delta_2+1}{2}$, a larger gap between the first and the second largest degrees in the network results in a more secure system, i.e., lower system $\mathcal{H}_2$ norm. In this sense, the most secure network topology would be the star graph since in that case we have $\Delta_1=n-1$ and $\Delta_2=1$. Moreover, according to the above results, increasing the connectivity of the underlying network does not have an effect on the game value $J_1(\mathfrak{F},\mathfrak{D})$ in \eqref{eqn:objectives}.
\end{remark}
\fi

\subsection{Multiple Attacked-Multiple Defense Nodes}

Now consider the case that there exist $f$ attacked nodes and $f$ defense nodes, i.e., $|\mathfrak{F}|=|\mathfrak{D}|=f\geq 1$. Here we only consider a Stackelberg setup as it is more applicable to security problems \cite{Manshaie}. We remark that if the defender is the leader, it reflects the defender's need to consider the worst case. Thus, it is more convenient to have the defender as the game leader.  

The Stackelberg game is a combinatorial problem. Thus, in general, its computational cost would be high, unless it is reduced with specific assumptions.  With this in mind, in our problem, finding optimal defense nodes when the defender is the game leader is burdensome, unless the control gain $k$ is sufficiently large and the number of attacked nodes is sufficiently small. 

\begin{theorem}\label{thm:multistack}
Consider a Stackelberg attacker-defender game on $J_1(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives} where there exists $f$ attacked nodes and $f$ defense nodes, $f \geq 1$ and $n\geq 2f$, with the defender as the game leader.  If 
$k\geq \frac{1}{2}(fd_{\rm \max}-2)$ then at the equilibrium the defender chooses $v=\arg\max_{\substack{\mathfrak{D} \subseteq \mathcal{V}\\|\mathcal{D}|=f}} \sum_{v_i \in \mathfrak{D}}d_i$, i.e., $f$ nodes with the largest degrees in the network. The best response of the attacker is to choose $\bar{v}=\arg\max_{\substack{\mathfrak{F}\subseteq \mathcal{V}\setminus v\\|\mathcal{F}|=f}} \sum_{v_i \in \mathfrak{F}}d_i$.
\end{theorem}




\iffalse
It worth noting that, if the attacker is the leader of the Stackelberg game, without further assumption on the control gain $k$, the problem is computationally tractable. 

\begin{theorem}
Consider a Stackelberg attacker-defender game on $J_1(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives} with $f$ attacked nodes and $f$ defense nodes, $f \geq 1$, with the attacker as the game leader. Then at the equilibrium the attacker chooses  $v=\arg\max_{\mathfrak{F} \subseteq \mathcal{V}} \sum_{v_i \in \mathfrak{F}}d_i$, i.e., the $f$ nodes with largest degree in the network. In this case, the best response by the defender will be identical to the attacker.
\label{thm:skjg}
\end{theorem}
\fi






















\section{Attacker-Defender Game on $J_2(\mathfrak{F}, \mathfrak{D})$}
\label{sec:oegb}
In this section, we discuss the dynamics with control law \eqref{subeq1} and objective function $J_2(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives}. 


\subsection{Single Attacked, Single Defense Nodes}

Similar to the case of $J_1(\mathfrak{F}, \mathfrak{D})$, we start with the case of  single attacked and  single defense nodes. We first have the following proposition.
\begin{proposition}
The  attacker-defender game on $J_2(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives}  with a single attack and single defense node does not admit an NE. \label{prop:none}
\end{proposition}

Similar to the attacker-defender game on $J_1(\mathfrak{F}, \mathfrak{D})$, in the absence of NE, an optimal defense strategy can be determined by finding the solution of the Stackelberg game.
Recalling the notion of the {\it effective center of a graph}, from Section \ref{sec:not}, we have the following theorem which is proven in Appendix \ref{sec:thm44}.
\begin{theorem}\label{thm:complexx}
Consider the Stackelberg attacker-defender game on $J_2(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives} on graph $\mathcal{G}$ with the defender as the game leader.  Then, a solution of the game corresponds to the case when the defender chooses the effective center of  $\mathcal{G}$, i.e., $\mathfrak{D}^*=\arg\min_{v \in \mathcal{V}}\epsilon_f (v)$. In this case, the best response of the attacker will be $\mathcal{B}^*(\mathfrak{D})=\arg\max_{j\in \mathcal{V}}R_{\mathfrak{D}^*j}$, i.e., a node with the maximum effective resistance from $\mathfrak{D}^*$.
\end{theorem}

For the case of acyclic networks, Theorem \ref{thm:complexx} reduces to the following corollary.

\begin{corollary}[\textbf{Acyclic Networks}]\label{cor:costfew}
Consider the Stackelberg attacker-defender game on $J_2(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives}, with the defender as the game leader, over the connected undirected tree $\mathcal{G}$.  At equilibrium,  the defender chooses the  {\it center} of the graph and the attacker chooses the node with the greatest distance from the center. 
\end{corollary}


\begin{remark}[\textbf{Game Equilibriums and Network Centrality}]\label{rem:ssodjnf}
As mentioned before, the optimal location of the defense node for the objective function $J_1(\mathfrak{F}, \mathfrak{D})$ is the degree central node (Theorem \ref{thm:necsuefgame})  and for $J_2(\mathfrak{F}, \mathfrak{D})$ is the graph's center for acyclic networks (Corollary \ref{cor:costfew}) or effective center for general graphs (Theorem \ref{thm:complexx}). These network centralities (and consequently optimal defense node placements) can differ substantially from each other. One of such examples is the graph shown in Fig.~\ref{fig:center1} (a), in which by increasing the length of the  path, the two centralities become far apart.
\end{remark}




\begin{figure}[t!]
\centering
\includegraphics[scale=.4]{centers.pdf}
\caption{(a) Optimal locations of the defense node for objective functions $J_1(\mathfrak{F}, \mathfrak{D})$ and $J_2(\mathfrak{F}, \mathfrak{D})$, (b) Extended graph and the virtual agent (ground). }
\label{fig:center1}
\end{figure}





























\iffalse
\section{Equilibrium Analysis: Multiple Attack Nodes, Single defense Node On Trees}
In this section, we analyze the attacker-defender game with multiple attack nodes and a single defense node. One can interpret this as the lack of knowledge about the number of attacks to the network. In this case, if the defender knows an upper bound on the number of attacks $f$, then it can choose a strategy  which corresponds to the worst case scenario, i.e.,  $f$ nodes are under attack. The following remark discusses this worst case more formally.
\begin{remark}\textbf{(Effect of Adding Attackers)}:
By increasing the number of attackers, the game payoff  will increase (the energy required to attack the system will decrease). More formally, since $\bar{L}^{-1}$ is a positive matrix,  for two attack sets $\mathcal{B}$ and $\bar{\mathcal{B}}$ where ${\mathcal{B}}\subseteq \bar{\mathcal{B}}$ , we have $\sum_{i\in \mathcal{B}}[\bar{L}^{-1}]_{ii} \leq \sum_{i\in \bar{\mathcal{B}}}[\bar{L}^{-1}]_{ii}$.
\end{remark}

For this scenario, the optimal strategy of the single defender depends on the number of nodes under attack. 
The following theorem characterizes the equilibrium solution of the game with multiple attack nodes and a single defense node. The proof of this theorem follows a similar procedure to that of Theorem \ref{thm:complexx}. The notion of graph's $f$-center was defined in Section \ref{sec:not}.
\begin{theorem}\label{thm:costsfew}
Consider the Stackelberg attacker-defender game with single defender and  $f$ attacks, $f>1$, with the defender as the game leader, over the connected undirected tree $\mathcal{G}$.  Then, a solution of the game is when the defender chooses the weighted $f$-center of the graph and the attackers choose the farthest $f$ nodes from the $f$-center.
\end{theorem}
It should be noted that the graph's closeness central node (the node whose summation of its distances to all other nodes is minimized) is equivalent to $(n-1)$-center node. In general, the location of graph's $f$-center in the network changes by changing $f$. This is discussed in the following example. 

\begin{example}
A broom tree is a graph which is formed by a star, comprised of $m$ nodes connected to the center, followed by a tail of length $m$. In the broom tree shown in Fig. \ref{fig:1} (a), the closeness central node of the graph always is in the center of the star; however, the center (and in general its $f$-center) will go left through the tail as $m$ increases. 
\begin{figure}[t!]
\centering
\includegraphics[scale=.33]{broomexample.pdf}
\caption{An example of a graph showing that the $f$-center of a graph can change with $f$.}
\label{fig:1}
\end{figure}
\label{exp:egewg}
\end{example}

Theorem \ref{thm:costsfew} together with Example \ref{exp:egewg} show that in the absence of knowledge of the number of attacks on the system, choosing one of $f$-centers of the graph results in a sub-optimal solution. However, it gives a message that  centralities which are distance-based (like $f$-centrlities mentioned above) are among appropriate choices for the defender. In other words, degree-based centralities, such as degree central node and eigenvector central node \cite{Newman_Networks_Book}, can reach to inappropriate decisions, as discussed in the following example.

\begin{example}
In Fig. \ref{fig:1} (b), the degree and eigenvector central nodes are the two nodes in the end of the  path; however, the $f$-central node, for any $f\leq n-1$,  is located in the middle of the  path. By increasing the length of the  path, the  $f$-central node becomes  arbitrarily far from the degree (and eigenvector) central nodes. 
\end{example}
\fi







\subsection{Multiple Attacked, Multiple defense Nodes}\label{sec:effectaafdd}


In order to tackle this problem, we interpret the self-feedback loops in the form of connections to  some virtual agent (or grounded node) as shown in Fig. \ref{fig:center1} (b). In this case, matrix $\bar{L}$ would be  a submatrix of the Laplacian matrix $L_{(n+1)\times (n+1)}$ of the extended graph (including $\ell$) where the row  and the column corresponding to $\ell$ are removed. Such submatrices are called grounded Laplacian in the literature \cite{ArxiveRobutness}. With this is mind, it is known that the $i$-th diagonal element of $\bar{L}^{-1}$ is $R_{i\ell}$, i.e., the effective resistance between node $v_i$ and the virtual node $\ell$ \cite{Ghosh2008}.\footnote{When the graph is a tree, the effective resistance and physical distance become the same.}
As an example, consider nodes 1 and 2 in Fig.~\ref{fig:center1} (b) which are chosen as defenders and nodes 1 and 3 which are under attack. In this case, we have $J_2(\mathfrak{F},\mathfrak{D})=1+\frac{1}{2}\sum_{i\in \mathfrak{F}}\bar{L}^{-1}_{ii}=1+\frac{1}{2}(R_{1\ell}+R_{3\ell})$. Based on this fact, the proof of the  following theorem is straightforward.
\begin{theorem}\label{thm:complex}
Consider the Stackelberg attacker-defender game on $J_2(\mathfrak{F}, \mathfrak{D})$ in \eqref{eqn:objectives} with $f$ defense nodes and  $f$ attack nodes, $f\geq 1$, with the defender as the game leader, over the connected undirected graph $\mathcal{G}$.  Denote the virtual agent corresponding to a set of $f$ defense nodes $\mathfrak{D}$ by $\ell_{\mathfrak{D}}$. Then, a solution of the game is when the defender chooses set $\mathfrak{D}$ in which the maximum sum of effective resistances between $\ell_{\mathfrak{D}}$ and all combinations of $f$ nodes in the network is minimized, i.e., $\mathfrak{D}^*=\arg\min_{\mathfrak{D}\subseteq \mathcal{V}}\max_{\mathfrak{F}\subseteq \mathcal{V}}\sum_{j\in \mathfrak{F}}R_{\ell_{\mathfrak{D}}j}$. In this case, the attacker chooses the set of $f$ attacked nodes as $\mathfrak{F}^*=\arg\max_{\mathfrak{F}\subseteq \mathcal{V}}\sum_{j\in \mathfrak{F}}R_{\ell_{\mathfrak{D}^*}j}$. 
\end{theorem}

As it is seen from Theorem \ref{thm:complex}, finding the optimal set of defense nodes  requires a high level of computation. 

\begin{remark}\textbf{(The Effect of Increasing Connectivity)}:
Since the effective resistance between two nodes in the graph is an increasing function of edge weights  \cite{ArxiveRobutness}, adding extra edges to the network (or increasing the weight of edges)  decreases the diagonal elements of $\bar{L}^{-1}$ and consequently decreases the system $\mathcal{H}_2$ norm. Hence, unlike control law \eqref{subeq2}, increasing connectivity is beneficial from the defender's perspective for \eqref{subeq1}.
\label{rem:1s}
\end{remark}


\iffalse
The following remark discusses the effect of adding a defense node on the game value.
\begin{remark}\textbf{(The Effect of Adding defense nodes)}:
In the extended graph, adding a self-feedback loop to node $v_i$ is equivalent to adding an edge from $v_i$ to the virtual agent with weight $k$. Hence, similar to what was discussed in Remark \ref{rem:1s}, adding extra defense node results in decreasing the game value; thus, it is beneficial for the security of the system.
\end{remark}
\fi















\iffalse



\subsection{Attack Model}

 
To examine the resilience of the dynamic \eqref{eqn:partial}  against cyber-physical attacks, we assume that an attacker injects attack signals to  a set of nodes in the network. Let $\mathcal{B}$ denote the set of nodes under attack. Thus, the dynamic of the node $v_i \in \mathcal{B}$ will evolve according to
  \begin{equation}
\dot{x}_i(t)=\sum_{j\in \mathcal{N}_i}w_{ij}\left(x_j(t)-x_i(t)\right)-k\left(x_i(t)-x_i(0)\right)+\zeta_i(t),
 \end{equation}
 where $\zeta_i(t)$ represents the attack signal on node $v_i$. In this paper we assume that $\zeta_i(t)=\zeta(t)$, $\forall i\in \mathcal{B}$. 
 Aggregating the dynamics of agents into a matrix form yields the following linear time-invariant network dynamical system
\begin{align}
\dot{\boldsymbol x}(t) &= -\bar{L}\boldsymbol x(t) + K\boldsymbol x(0)+B\boldsymbol \zeta(t),
\label{eqn:partial4}
\end{align}
where matrix $B=[\textbf{e}_1, \textbf{e}_2, ..., \textbf{e}_f]$ specifies the selected nodes by attacker. Note that the attacker selects the columns of the matrix $B$ and the value of the attack signal $\boldsymbol \zeta (t)$ is not a decision variable. We assume that the value of the feedback parameter $k$ is private and is unknown to the attacker.\footnote{ Otherwise the attacker can choose $\zeta_i(t)=k\left(x_i(t)-x_i(0)\right)$ and makes the defender as an ordinary agent. }  

In the presence of an attack, dynamics \eqref{eqn:partial4}  can be potentially deviated from the convex hull of the initial conditions, unless the underlying network is sufficiently connected \cite{dibaji2017resilient, Hogan, Leblankk}. However, having a highly connected network is a demanding condition for many applications. In this case, we have to adopt an alternative strategy to prohibit or mitigate the effect of the attack even when the underlying network topology is sparse as it will be discussed in the following subsection.

\section{Attacker-Defender Game}
In this section, we propose a game-theoretic framework for designing secure consensus algorithms. More formally, we pose the problem as a zero-sum game between an attacker  and a defender. The objective of the game is the  system $\mathcal{H}_2$ norm from the attack signals to the deviation of generators frequencies from the nominal value.  The attacker selects a set of network nodes, to inject the attack signals, such that system $\mathcal{H}_2$ norm is maximized. The defender selects a set of nodes to place self-feedback loops such that this system norm is minimized.  Mathematically speaking, the decision variable of the attacker is matrix $B$ and the decision variable of the defender is matrix $D_y$. The notion of average energy here is captured by the trace of the controllability Gramian matrix, associated with the dynamics in \eqref{eqn:partial4}, which can be written as  
\begin{equation}
\mathcal{W}_c=\int_0^{\infty} \mathbf{e}^{\bar{L}\tau}BB^T\mathbf{e}^{\bar{L}^T\tau}d\tau.
\end{equation}
Based on the following calculations, the trace of the controllability Gramian of \eqref{eqn:partial4} has a closed form 
\begin{align}
\trace\left(\mathcal{W}_c\right)&=\trace\left(\int_0^{\infty} \mathbf{e}^{\bar{L}\tau}BB^T\mathbf{e}^{\bar{L}^T\tau}d\tau\right)\nonumber\\
&=\int_0^{\infty} \trace\left( B^T\mathbf{e}^{2\bar{L}\tau}B\right)d\tau= \trace\left( B^T\int_0^{\infty}\mathbf{e}^{2\bar{L}\tau}d\tau B\right)\nonumber\\
&= \frac{1}{2}\trace \left(B^T\bar{L}^{-1}B\right)=\sum_{i\in \mathcal{B}}[\bar{L}^{-1}]_{ii},
\end{align}
where $[\bar{L}^{-1}]_{ii}$ is the $i$-th diagonal element of  $\bar{L}^{-1}$. Based on the above closed form, the following game is defined. 
 \begin{tcolorbox}
\textbf{Attacker and Defender Game:} The attacker tries to inject attack signal $\zeta_i(t)$ to $f$ nodes in the network to maximize the average controllability $\trace \left(\mathcal{W}_c\right)$, while the defender places the self feedbakcs to $f$ nodes to minimize the average controllability of the system. Thus the game payoff for this attacker-defender zero-sum game is:
\begin{align}\label{eqn:objectives}
J(B, D_y)&=\frac{1}{2}\trace \left(B^T(\underbrace{L+kD_y}_{\bar{L}})^{-1}B\right),
\end{align}
where the attacker's decision determines matrix $B$ to maximize $J(B, D_y)$ and the defender's decision affects matrix $D_y$ to minimize $J(B, D_y)$.
\end{tcolorbox}

Fig.~\ref{fig:leadesr} shows an example of the attacker defender game. Based on this figure, the attacker chooses nodes 1 and 3, while the defender chooses nodes 1 and 2. Based on the actions of the attacker and the defender, matrix game $A$ is formed where the attacker (maximizer) chooses columns and the defender (minimizer) chooses the rows. In this case the game value is $a_{12}=\bar{L}_{11}^{-1}+\bar{L}_{33}^{-1}$.
\begin{figure}[t!]
\centering
\includegraphics[scale=.4]{attackdef.pdf}
\caption{An example of the attacker-defender game.}
\label{fig:leadesr}
\end{figure}
Through the rest of the paper we investigate the equilibrium of the above game for the case of single (and multiple) attacker and defender. Note that the equilibrium strategy of the game determines the optimal location of self-feedback loops.
\begin{remark}
It is known that optimizing the trace of controllability Gramian does not preserve the controllability of the system, e.g., having $\mathcal{W}_c \succ 0$ \cite{Pasqualetti}. If minimizing $\trace (\mathcal{W}_c)$ (from defender's perspective) yields to an uncontrollable system, then the action of the defender can be interpreted as maximizing the energy of steering the system  over the {\it controllable subspace}, which is the range space of $\mathcal{W}_c$. 
\end{remark}


















\section{Equilibrium Analysis: Single Attack Single defense Nodes On Trees}

In this section, we investigate the attacker-defender game when the attacker and the defender choose  single nodes  and the underlying network is a tree. The reason of choosing trees is that it provides insights about the role of  network topology on the game strategy. We will discuss more general graphs in Section \ref{sec:effectaafdd}.


For the single attack-single defense nodes case, the game payoff will simply become 
\begin{equation}
J(B, D_y)=[(L+k\mathbf{e}_j\mathbf{e}_j^T)^{-1}]_{ii},
\end{equation}
where $v_i$, and $v_j$ are the node under attack and the node with the self-feedback, respectively. We need the following lemma to further study the game value and the equilibrium strategies.  The proof of this lemma is postponed to Section \ref{sec:effectaafdd}.

\begin{lemma}\label{lem:treehinf}
Suppose that $\mathcal{G}$ is an undirected tree and there exists a single defense node  $v_j$ (which has a self loop with weight $k$). Then  we have
\begin{equation}
   [\bar{L}^{-1}]_{ii}=\frac{1}{k}+ \sum_{h\in \mathcal{P}_{ij}}\frac{1}{w_h},
\end{equation}
where $\mathcal{P}_{ij}$ is the set of nodes in the (unique) path from $v_i$ to $v_j$.
\end{lemma}

We next show that the attacker defender game does not admit an NE. 
\begin{proposition}
The single attacker-single defender game with a single attack and single defense node does not admit an NE.
\end{proposition}
\begin{proof}
The proof is based on the fact that the value of all diagonal elements of the game matrix $A$ is $A_{ii}=\frac{1}{k}$ and each off-diagonal element is $A_{ij}=\frac{1}{k}+ \sum_{h\in \mathcal{P}_{ij}}\frac{1}{w_h}$. Thus, each diagonal element is strictly less than the elements of its corresponding row and column. Now assume that a NE exists and let $(i^*,j^*)$ denote the equilibrium strategies of the attacker and defender. Thus, we should have
 \begin{equation}\label{eqn:sdgjb}
[A]_{i^*j}\leq [A]_{i^*j^*}\leq [A]_{ij^*}
\end{equation}
for all $i\neq i^*$ and $j\neq j^*$. 
If element $[A]_{i^*j^*}$ is in one of the diagonal elements then the left inequality will be violated and if it is in one of the non-diagonal elements, the right inequality will be violated. 
\end{proof}

Although the attacker-defender game does not admit an NE, the optimal defense strategy can be determined by finding the solution of the Stackelberg game between the attacker and defender.  
In the Stackelberg game formulation, the defender acts as the game leader, \emph{i.e.,} the leader solves the following optimization problem
\begin{equation}\label{eqn:stackd}
J^*(D_y)=\min_{D_y}\trace \left(B^{*^T}(D_y)\bar{L}^{-1}B^*(D_y)\right).
\end{equation}
where $D_y$ is chosen over all $f$ defense nodes (here $f=1$) in $\mathcal{V}$ and $B^*(D_y)$ is the best response of the attacker when the strategy of the defender is $D_y$, i.e., $B^*(D_y)$ is the solution of the following optimization problem
\begin{equation}\label{eqn:stack}
B^*(D_y)=\arg\max_B\trace \left(B^{T}\bar{L}^{-1}B\right),
\end{equation}
where $B$ is chosen over all ${f}$ attacked nodes (here ${f}=1$) in $\mathcal{V}$.
In particular, for a given strategy of the defender, i.e., $D_y$, the attacker finds its best response strategy to the defender's decision, which is given by $\arg\max_B\trace \left(B^{T}\bar{L}^{-1}B\right)$. Then, the defender optimizes its decision based on all possible best response strategies of the attacker. 

%Before discussing the Stackelberg game result, we present the following definitions.
%\begin{definition}[\cite{Harary}]\textbf{(Eccentricity
%and Graph Center)}:
%The eccentricity $\epsilon (v)$ of a vertex $v$ in a connected weighted graph $\mathcal{G}$ is the maximum graph distance (or weighted distance) between $v$ and any other vertex $u$ of $\mathcal{G}$. The center of a graph is a set of vertices with minimum (weighted) eccentricity. 
%\end{definition}

Based on the above discussion and the definition of graph center presented in Section \ref{sec:not}, we have the following theorem.
%\begin{theorem}\label{thm:costfew}
Consider the Stackelberg attacker-defender game, with the defender as the game leader, over the connected undirected tree $\mathcal{G}$.  Then, a solution of the game corresponds to the case when the defender chooses the weighted center of the graph and the attacker chooses the node with longest (weighted) distance from the center. 
%\end{theorem}
\begin{proof}
We know that for the  game matrix $A$ we have  $A_{ij}=\frac{1}{k}+ \sum_{h\in \mathcal{P}_{ij}}\frac{1}{w_h}$. As the defender is the leader of the Stackelberg game, it minimizes (over all rows) the maximum element of each row of $A$. Since the term $\frac{1}{k}$ is shared over all elements of $A$, then the optimal place for the defender is $v^*=\arg\min_{i}\max_{j}\sum_{h\in \mathcal{P}_{ij}}\frac{1}{w_h}$ and this is the center of the graph, whose (weighted) eccentricity is minimized.  Note that this solution (strategies of the defender and attacker) may not be unique since the center of the network may not be a single node. However, the value of the game is unique.
\end{proof}





\section{Equilibrium Analysis: Multiple Attack Nodes, Single defense Node On Trees}
In this section, we analyze the attacker-defender game with multiple attack nodes and a single defense node. One can interpret this as the lack of knowledge about the number of attacks to the network. In this case, if the defender knows an upper bound on the number of attacks $f$, then it can choose a strategy  which corresponds to the worst case scenario, i.e.,  $f$ nodes are under attack. The following remark discusses this worst case more formally.
\begin{remark}\textbf{(Effect of Adding Attackers)}:
By increasing the number of attackers, the game payoff  will increase (the energy required to attack the system will decrease). More formally, since $\bar{L}^{-1}$ is a positive matrix,  for two attack sets $\mathcal{B}$ and $\bar{\mathcal{B}}$ where ${\mathcal{B}}\subseteq \bar{\mathcal{B}}$ , we have $\sum_{i\in \mathcal{B}}[\bar{L}^{-1}]_{ii} \leq \sum_{i\in \bar{\mathcal{B}}}[\bar{L}^{-1}]_{ii}$.
\end{remark}

For this scenario, the optimal strategy of the single defender depends on the number of nodes under attack. 
The following theorem characterizes the equilibrium solution of the game with multiple attack nodes and a single defense node. The proof of this theorem follows a similar logic to that of Theorem \ref{:costfew}. The notion of graph's $f$-center was defined in Section \ref{sec:not}.
\begin{theorem}\label{thm:costsfew}
Consider the Stackelberg attacker-defender game with single defender and  $f$ attacks, $f>1$, with the defender as the game leader, over the connected undirected tree $\mathcal{G}$.  Then, a solution of the game is when the defender chooses the weighted $f$-center of the graph and the attackers choose the farthest $f$ nodes from the $f$-center.
\end{theorem}
It should be noted that the graph's closeness central node (the node whose summation of its distances to all other nodes is minimized) is equivalent to $(n-1)$-center node. In general, the location of graph's $f$-center in the network changes by changing $f$. This is discussed in the following example. 

\begin{example}
A broom tree is a graph which is formed by a star, comprised of $m$ nodes connected to the center, followed by a tail of length $m$. In the broom tree shown in Fig. \ref{fig:1} (a), the closeness central node of the graph always is in the center of the star; however, the center (and in general its $f$-center) will go left through the tail as $m$ increases. 
\begin{figure}[t!]
\centering
\includegraphics[scale=.33]{broomexample.pdf}
\caption{An example of a graph showing that the $f$-center of a graph can change with $f$.}
\label{fig:1}
\end{figure}
\label{exp:egewg}
\end{example}

Theorem \ref{thm:costsfew} together with Example \ref{exp:egewg} show that in the absence of knowledge of the number of attacks on the system, choosing one of $f$-centers of the graph results in a sub-optimal solution. However, it gives a message that  centralities which are distance-based (like $f$-centrlities mentioned above) are among appropriate choices for the defender. In other words, degree-based centralities, such as degree central node and eigenvector central node \cite{Newman_Networks_Book}, can reach to inappropriate decisions, as discussed in the following example.

\begin{example}
In Fig. \ref{fig:1} (b), the degree and eigenvector central nodes are the two nodes in the end of the  path; however, the $f$-central node, for any $f\leq n-1$,  is located in the middle of the  path. By increasing the length of the  path, the  $f$-central node becomes  arbitrarily far from the degree (and eigenvector) central nodes. 
\end{example}








\section{Multiple Attack, Multiple defense Nodes on General Graphs}\label{sec:effectaafdd}


In this section, we discuss the case where there are $f$ attack and $f$ defense (self-feedback loops) in the general network where $f ,f \geq 1$. In order to tackle this problem, we need to reinterpret the self-feedback loops in terms of connections to some virtual agent as shown in Fig. \ref{fig:leader}.
\begin{figure}[t!]
\centering
\includegraphics[scale=.4]{leader.pdf}
\caption{Extended graph and the virtual leader.}
\label{fig:leader}
\end{figure}
We call the graph including such a virtual agent the {\it extended graph} and its Laplacian is denoted by ${L}_{ext}$. Any defense node is connected to that virtual agent with an edge of weight $k$ (the self-feedback). This virtual agent is interpreted as a grounded node if we interpret the network as a circuit. Thus, it does not have any effect on the dynamics and exists only to facilitate the graph-theoretic interpretation of the attacker-defender game. 

Here we relax the assumption of acyclic networks and solve the game on general graphs. In this case, as there may be multiple paths between each couple of nodes, each element of the game matrix $a_{ij}$ will be the sum of effective resistances (instead of the physical distance) between nodes in the $i$-th attack set (consists of $f$ attacks) when the node set $j$ (consists of $f$ defenders) is chosen to be the defender set. %The notion of effective resistance is defined bellow. 

%\begin{definition}
 %The {\it effective resistance}, $R_{ij}$, between two vertices $v_i$ and $v_j$ in a graph is the equivalent resistance between these two vertices when we treat the resistance of each edge $e$ as $\frac{1}{w_e}$, where $w_e$ is its weight. 
% \end{definition}

%Considering the above definition of the effective resistance, 
If we treat $\bar{L}$ as a grounded Laplacian matrix (grounded at the virtual node $\ell$), it is known that its $i$-th diagonal element is the effective resistance between node $v_i$ and the virtual node $\ell$ \cite{ArxiveRobutness}. \footnote{When the graph is a tree, the effective resistance and physical distance become the same and this proves the statement of Lemma \ref{lem:treehinf}.}
With this in mind, consider nodes 1 and 2 in Fig.~\ref{fig:leader} which are chosen as defenders and nodes 1 and 3 which are under attack. In this case, element $a_{12}$ in matrix game $A$ determines the game value which is equal to $a_{12}=\sum_{i\in \mathcal{B}}[\bar{L}^{-1}]_{ii}=R_{1\ell}+R_{3\ell}$. Based on this fact, the following theorem discusses the equilibrium of Stackelberg game for general case of $f$ attack nodes and $f$ defense nodes on connected undirected networks. 
\begin{theorem}\label{thm:complex}
Consider the Stackelberg attacker-defender game with $f$ defense nodes and  $f$ attack nodes, $f \geq 1$, with the defender as the game leader, over the connected undirected graph $\mathcal{G}$.  Let's denote the virtual agent corresponding to a set of $f$ defense nodes $\mathfrak{D}$ by $\ell_{\mathfrak{D}}$. Then, a solution of the game is when the defender chooses $f$ nodes $\mathfrak{D}$ in which the summation of effective resistances between $\ell_{\mathfrak{D}}$ and all combinations of $f$ nodes in the network is minimized, i.e., $\mathfrak{D}^*=\arg\min_{\mathfrak{D},\mathcal{B}\subseteq \mathcal{V}}\sum_{j\in \mathcal{B}}R_{\ell_{\mathfrak{D}}j}$. Moreover, the attacker chooses the set of $f$ attack nodes as $\mathcal{B}^*(\mathfrak{D})=\arg\max_{\mathcal{B}\subseteq \mathcal{V}}\sum_{j\in \mathcal{B}}R_{\ell(\mathfrak{D}^*)j}$.
\end{theorem}

As it is seen from Theorem \ref{thm:complex}, finding the optimal set of defense nodes consumes a high level of computation. There may be heuristic algorithms to tackle this problem with lower computational cost which are left for future research.
The following remark discusses the effect of increasing the connectivity on the security against the attacker's actions. 

\begin{remark}\textbf{(The Effect of Increasing Connectivity)}:
Since the effective resistance between two nodes in the graph is an increasing function of edge weights (or decreasing function of edge conductance, as mentioned in \cite{Ghosh2008}), adding extra edges to the network (or increasing the weight of edges) will  decrease the diagonal elements of $\bar{L}^{-1}$ and consequently decreases the trace of the controllability Gramian which results in increasing the attack energy. Hence, it would be beneficial from the defender's perspective.
With the same reasoning, removing edges (or weights) from the network results in a less secure system.
\label{rem:1s}
\end{remark}

The following remark discusses the effect of adding a defense node on the game value.
\begin{remark}\textbf{(The Effect of Adding defense nodes)}:
In the extended graph, adding a self-feedback loop to node $v_i$ is equivalent to adding an edge from $v_i$ to the virtual agent with weight $k$. Hence, similar to what was discussed in Remark \ref{rem:1s}, adding extra defense node results in decreasing the game value; thus, it is beneficial for the security of the system. 
\end{remark}

\section{Simulations}

In this section, we present simulation results for an attacker-defender game over a graph with single attack-single defense nodes. Fig. \ref{fig:leadsdfer} (top) shows the game payoffs for four sample defense nodes (nodes 8, 9, 10, and 11) each of which for all possible choices of the attack nodes (the horizontal axis belongs to the attacker's label).  
\begin{figure}[t!]
\centering
\includegraphics[scale=.40]{simulation.pdf}
\caption{single attacker-single defender, (Top) Effect of choosing the center of the graph as the defender, (b) comparing degree-based centralities with the center of the graph.}
\label{fig:leadsdfer}
\end{figure}
According to this figure, the best response of the attacker to each strategy of the defender  is to select the end of the  path (node 15) as the attack node. Thus, the optimal value from the defender's perspective (leader of the Stackelberg game) is to choose node 11 whose attacker's best response (node 15) is less than the other four (black star in node 15).  As another example, we look at the structure which was discussed in  Fig. \ref{fig:leader} as well where there are two stars linked with a  path. In this case, similar to the previous example, the game payoff for three sample nodes (6, 7, and 8) as defenders is depicted for all possible choices of the attack nodes (horizontal axis) and the best response of the attacker is node 1. \footnote{The best attacker's response it not unique since nodes 2 and 3 are also best responses.} Hence, the minimum of these values belongs to the case where the defender is located in node 6 and node 8 (regardless of its degree) would not be the solution of the Stackelberg game. 

The effect of choosing the network's 2-center for the defender when there exists two attack nodes is shown in Fig. \ref{fig:leadsddffer}. As shown in this figure, nodes 3 and 4 are chosen as two examples. Node 3, which is the 2-center of the graph, minimizes the best response of the attacker, compared to node 4, which is the center of the graph. 
\begin{figure}[t!]
\centering
\includegraphics[scale=.36]{simulation2.pdf}
\caption{Single defender and two attackers. Effect of choosing graph's 2-center.}
\label{fig:leadsddffer}
\end{figure}










\fi

==> CDC2019 (3)/extra_results.tex <==

\begin{definition}\textbf{(Resistance Distance):}
 The  resistance distance $\mathfrak{R}_{ij}$ between two vertices $v_i$ and $v_j$ in an undirected graph is the equivalent resistance between these two vertices when we treat each edge of the graph as a $1 \Omega$ resistor. \label{def:sldigub}
 \end{definition}

 For the resistance distance $\mathfrak{R}_{i,j}$ and the minimum physical distance between two nodes $\mathfrak{D}_{i,j}$, we have $\mathfrak{R}_{i,j}\leq \mathfrak{D}_{i,j}$, with equality if there exists one path between $v_i$ and $v_j$. Moreover, it can be shown that the resistance distance between $v_{\ell}$ and $v_j$ is the $j$-th diagonal element of $\mathcal{L}_{g{\ell}}^{-1}$, where $v_{\ell}$ is a single grounded vertex \cite{Bapat}. 




\begin{theorem}\label{thm:upperresis}
Consider a connected undirected graph $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ with a set of leaders $\mathfrak{S} \subset \mathcal{V}$.  Let $\mathcal{L}_g$ be the grounded Laplacian matrix induced by $\mathfrak{S}$. Then for the $\mathcal{H}_{\infty}$ norm of \eqref{eqn:partial4} for $\mathcal{B}=\mathbf{e}_i$ and $\mathcal{C}=\mathbf{e}_j^T$ we have
\begin{align}\label{eqn:roofad}
||G||_{\infty} \leq \min\{\min_{\ell \in \mathfrak{S}} \mathfrak{R}_{i,\ell}, \min_{\ell \in \mathfrak{S}}\mathfrak{R}_{j,\ell}\},
\end{align}
with equality when  $i=j$ and $|\mathfrak{S}|=1$.
\end{theorem}
\begin{proof}
The proof is based on the fact that 2-tree $t_{ij,\ell \ell}$ is also a 2-tree $t_{ii,\ell \ell}$, but the inverse is not true. Hence, the cardinality of set of 2-trees $t_{ii,\ell \ell}$ is larger than that of $t_{ij,\ell \ell}$. As a result, based on Lemma \ref{lem:jlsdhav} we conclude that $[\mathcal{L}^
{-1}]_{ij}\leq \min\{[\mathcal{L}^
{-1}]_{ii}, [\mathcal{L}^
{-1}]_{jj}\}$ and based on Definition \ref{def:sldigub} the result is obtained. 

The equality for the case where $i=j$ and there is a  single leader, $\ell$, is clear due to the fact that  $[\mathcal{L}_{g}^{-1}]_{ii}=\mathfrak{R}_{i,\ell}$. however, if $i=j$ and we add more leaders, their effects are considered by diagonal matrix $E=\sum_{k\in \mathcal{V}}\Gamma_k\mathbf{e}_k\mathbf{e}_k^T$, where  $\Gamma_k$ is the number of leaders connected to follower $v_k$. Then, for each matrix $\mathbf{e}_k\mathbf{e}_k^T$ we use Sherman-Morrison formula to get
\begin{align}\label{eqn:vnoswfup}
\Tilde{\mathcal{L}}_{g}^{-1}=\left( \mathcal{L}_{g} + \mathbf{e}_k\mathbf{e}_k^T \right)^{-1}=\mathcal{L}_{g}^{-1}-\frac{\mathcal{L}_{g}^{-1}\mathbf{e}_k\mathbf{e}_k^T\mathcal{L}_{g}^{-1}}{1+\mathbf{e}_k^T\mathcal{L}_{g}^{-1}\mathbf{e}_k}.
\end{align}
Based on the fact that $\mathcal{L}_{g}^{-1}$ is a nonnegative matrix, we conclude from \eqref{eqn:vnoswfup} that the elements of $\tilde{\mathcal{L}}_{g}^{-1}$ will be not larger than those of $\mathcal{L}_{g}^{-1}$, so as its diagonal elements, and this proves the claim. 
\end{proof}

Clearly, when the underlying graph is a tree, based on Theorem \ref{thm:upperresis} we have $||G||_{\infty} \leq \min\{\min_{\ell \in \mathfrak{S}} \mathfrak{D}_{i,\ell}, \min_{\ell \in \mathfrak{S}}\mathfrak{D}_{j,\ell}\}$ with equality if $i=j$ and $|\mathfrak{S}|=1$. The bound mentioned in Theorem \ref{thm:upperresis} are loose in some cases. One of such examples is shown in Fig. \ref{fig:sstdvqwefnj}. In this figure, which is a tree, we have $\mathfrak{R}_{i\ell}=\mathfrak{R}_{j\ell}=3$, while $[\mathcal{L}^
{-1}]_{ij}=1$. 





















\subsection{Mixed Strategy}

For the case of mixed strategy, as stated in Lemmas \ref{lem:blaiug} and \ref{lem:puremix}, upper and lower bounds on the value of the game were proposed. In the context of our case study which is the leader-follower dynamics on trees, we apply these results. Moreover, we compare case of directed trees and undirected trees to examine reducible matrix $L_g^{-1}$ where we have equality $v(L_g^{-1})=\rho(L_g^{-1})$. More formally, we present the following theorem.

\begin{proposition}\label{prop:asjDB}
Let $\mathcal{G}$ be an undirected tree satisfying Assumption 1. Then for the value of mixed game we have $v(L_g^{-1})\geq 1$ and $v(L_g^{-1})> 1$ for complete mixed strategy.
\end{proposition}
\begin{proof}
According to Lemma \ref{lem:puremix} since we have $[L_g^{-1}]_{ij}\geq 1$ for all $i,j=1,2,...n-1$ for undirected trees, the result is proved.
\end{proof}
Based on the above proposition, we present the following important corollary.
\begin{corollary}\label{cor:mixedtreeee}
Let $\mathcal{G}$ be an undirected tree satisfying Assumption 1 and let $\Bar{\mathcal{G}}$ be the directed version of $\mathcal{G}$ with the leader as the source node, i.e., $d_{\rm in}^{\ell}=0$. If $v$ is the mix strategy value for undirected graph and $\Bar{v}$ is the mixed strategy value for directed graph. Then  $v(L_g^{-1})\geq \Bar{v}(L_g^{-1})$.
\end{corollary}
\begin{proof}
According to Proposition \ref{prop:asjDB} we have that $v(L_g^{-1})\geq 1$. However, for directed trees, according to Lemma \ref{lem:blaiug} since $L_g^{-1}$ is reducible we have $\Bar{v}(L_g^{-1})=\rho(L_g^{-1})$. On the other hand since $L_g^{-1}$ is triangular, we have $\rho(L_g^{-1})=\frac{1}{d_{\rm min}}=1$ which proves the claim. 
\end{proof}





 
 \iffalse
 
 
 
 \subsection{Mixed Strategy}
 As, according to Theorem \ref{thm:noequilibrium}, there is no saddle point equilibrium for the pure strategy, we look at the mixed strategy for which the detector and the attacker are choosing a node with a specific probability. More formally, the attacker chooses each node $v_i$ with probability $x_i$ to attack and the detector chooses node $v_i$ with probability ${y}_i$. Clearly $\sum_{i=1}^nx_i=\sum_{i=1}^ny_i=1$. The game is called complete mixed if $x_i,y_i>0$ for all $i=1, 2, ...,n$. For the mixed strategy, the average value of the outcome of the game, corresponding to the strategy pair $\{B,C\}$, will be equal to 
 \begin{equation}
    J(x,y)=\sum_{i=1}^n\sum_{j=1}^nx_i[A^{-1}]_{ij}y_j=\boldsymbol x^TA^{-1}\boldsymbol y,
 \end{equation}
 where $\boldsymbol x=[x_1, x_2, ..., x_n]^T$ and $\boldsymbol y=[y_1, y_2, ..., y_n]^T$ are probability distribution vectors. The attacker tends to minimize and the detector tries to maximize $J(x,y)$  by assigning probability distribution vectors $\boldsymbol x$ and $\boldsymbol y$, respectively. Unlike pure strategy, it is well-known that the mixed strategy always has a saddle point equilibrium, i.e., there are always $\boldsymbol x^*$ and $\boldsymbol y^*$ such that 
 \begin{equation}
\boldsymbol x^*^TA^{-1}\boldsymbol y\leq \boldsymbol x^*^TA^{-1}\boldsymbol y^*\leq \boldsymbol x^TA^{-1} \boldsymbol y^*, \forall \boldsymbol x \in \boldsymbol X, \boldsymbol x \in \boldsymbol Y.
 \end{equation}
 where $\boldsymbol X\triangleq \{\boldsymbol x\in \mathbb{R}^n:\boldsymbol x\geq 0, \sum_{i=1}^nx_i=1\}$, $\boldsymbol Y\triangleq \{\boldsymbol y\in \mathbb{R}^n:\boldsymbol y\geq 0, \sum_{i=1}^ny_i=1\}$.

Using the nonnegativity of $A^{-1}$, we introduce the following two lemmas which give some bounds on the mixed game value and will be used later in Section \ref{sec:netint}.
\begin{lemma}[\cite{Cohen}]\label{lem:blaiug}
For the value of the mixed single attacker-detector game on \eqref{eqn:attackmain} we have $v(A^{-1})\leq \rho(A^{-1})$ with equality if and only if $A^{-1}$ is a reducible matrix, where $\rho$ is the spectral radius of a matrix. 
\end{lemma}

 \begin{lemma}\label{lem:puremix}
 For the value of the mixed single attacker-detector game on \eqref{eqn:attackmain} we have  $v(A^{-1})\geq \max_i\min_j[A^{-1}]_{ij}$ with strict inequality if  the game is completely mixed.
\end{lemma}
\begin{proof}
Based on the definition we have $v(A^{-1})=\max_{\boldsymbol x}\min_{\boldsymbol y}\boldsymbol x^TA^{-1}\boldsymbol y$ for all $\boldsymbol x,\boldsymbol y\geq 0$ where $\mathbf{1}^T\boldsymbol x=\mathbf{1}^T\boldsymbol y=1$. We choose $\boldsymbol x=\textbf{e}_i$ where $i=\arg\max_i\min_j[A^{-1}]_{ij}$. This gives  
\begin{equation}
v(A^{-1})\geq \min_{\boldsymbol y}\textbf{e}_i^TA^{-1}\boldsymbol y= \min_{\boldsymbol y}[A^{-1}]_i\boldsymbol y\geq \max_i\min_j[A^{-1}]_{ij},
\label{eqn:aSEOJgb}
\end{equation} 
where $[A^{-1}]_i$ is the $i-$th row of $A^{-1}$. The right inequality in \eqref{eqn:aSEOJgb} is due to the fact that $\mathbf{1}^T\boldsymbol y=1$ which gives a convex combination of the elements of the $i-$th row of $A^{-1}$ which is not smaller than $\max_i\min_j[A^{-1}]_{ij}$. For the case of complete mixed game, i.e., $\boldsymbol y>0$, we have \eqref{eqn:aSEOJgb} as
\begin{align}
v(A^{-1}) \geq  \min_{\boldsymbol y}[A^{-1}]_i\boldsymbol y>\max_i\min_j[A^{-1}]_{ij}.
\end{align}
\end{proof}
 
In the following section, we will focus on a specific class of dynamics \eqref{eqn:attackmain}, called leader-follower dynamics.
 
 
 
 
 \fi
 
 
 
 
 %%%%%% General Metzler matrices
 
 
 Consider a network of agents $\mathcal{G}=\{\mathcal{V}, \mathcal{E}\}$ where each agent $v_i$ has a scalar and real valued state $x_i(t)$, where $t$ is the time index, and is able to communicate with its neighbors and update its state via the following dynamics 
 \begin{equation}\label{eqn:11}
\dot{x}_i(t)=-a_{ii}x_i(t)+\sum_{j\in \mathcal{N}_i}a_{ij}x_j(t),
 \end{equation}
 where $a_{ij}$s are some positive and constant weights. In addition to \eqref{eqn:11} the updating rule of each agent is prone to an intrusion (or attack). More particularly, there exists a set of attackers $\mathcal{A}$ which inject $f$ attack signals to $f$ nodes in the network. \footnote{The number of attackers in practice is unknown and we can assume $f$ is an upper bound for the number of attacks.}Hence, if the the dynamics of agent $v_i$ is influenced by an attacker, it will be in the following form 
  \begin{equation}
\dot{x}_i(t)=-a_{ii}x_i(t)+\sum_{j\in \mathcal{N}_i}a_{ij}x_j(t)+w_i(t),
 \end{equation}
 where $w_i(t)>0$ represents the attack signal. To detect the effect of attacks, a set of $f$ dedicated sensors (or detectors), denoted by $\mathcal{D}$, are considered, each of which is placed on a specific node, i.e., 
 \begin{equation}
y_i(t)=x_i(t) \quad {\rm if} \quad v_i\in \mathcal{D}.
 \end{equation}
Aggregating the dynamics of each agent into a matrix form results in the following linear time-invariant network dynamical system
 \begin{align}\label{eqn:attackmain}
\dot{\boldsymbol x}(t)&=A\boldsymbol x(t)+ B\boldsymbol w(t),\nonumber\\
\boldsymbol y(t)&=C\boldsymbol x(t),
 \end{align}
 where $\boldsymbol w(t)$ is a vector of exogenous attack signal and we assume that there exists a nonempty time interval $\tau$ such that $\boldsymbol w(t)> \mathbf{0}$, $\forall t\in \tau$. Clearly, matrices $B$ and $C$ are binary matrices such that $B_{n\times f}=[\textbf{e}_1, \textbf{e}_2, ..., \textbf{e}_f]$  and $C_{f\times n}=[\textbf{e}_1^T; \textbf{e}_2^T; ...; \textbf{e}_f^T]$. In words, there is a single 1 in the $i$-th row (column) of matrix $B$ ($C$) if the $i$-th node is under attack (has a measurement). We assume that $||B||_0 >0$, i.e., there exists at least one attack to the system. An example of such systems is shown in Fig.~\ref{fig:sstdnj}. In this example, a $2\times 2$ matrix is chosen by the attacker and the detector from $A^{-1}$ which is shown in bold. 
 
\begin{figure}[t!]
\centering
\includegraphics[scale=.38]{gamedesign.pdf}
\caption{An Example of an attacker-detector game with $f=2$.}
\label{fig:sstdnj}
\end{figure}

 In this paper we assume that matrix $A$ is chosen to be Hurwitz and $-A$ is Metzler, i.e., its off diagonal elements are nonpositive, and row and column diagonally dominant. Based on the fact that $-A$ is Hurwitz, $-A^{-1}$ will be nonnegative elementwise.  The following definition yields Theorem \ref{thm:metzlertheroem} which is required for the rest of the analysis. 
 \begin{definition}\textbf{(Positive Systems)}:
A linear system is called (internally) positive if and only if its state and output are non-negative for every non-negative input and every non-negative initial state.
\end{definition}
\begin{theorem}[\cite{Rantzer}]
A continuous time linear system $(A, B, C)$ is positive if and only if $A$ is a Metzler-matrix and $B$ and  $C$ are non-negative elementwise.  Moreover, for such a positive system with transfer function $G(s)=C(sI-A)^{-1}B$, the system $L_2$ gain, which is equal to $\mathcal{H}_{\infty}$ norm for LTI systems, will be 
\begin{equation} \label{eqn:l2gain}
\sup_{||\boldsymbol w||_2\neq 0} \frac{||\boldsymbol y||_2}{||\boldsymbol w||_2}=\sigma_n(G(0))=\sigma_n(-CA^{-1}B),
\end{equation}
where  $\sigma_{n}$ is the maximum singular value of matrix $G(0)$ and the $L_2$ norm of signal $\boldsymbol u$ is $||\boldsymbol u||_2^2\triangleq \int_0^{\infty}\boldsymbol u^T\boldsymbol u$.
\label{thm:metzlertheroem}
\end{theorem}
 
Based on Theorem \ref{thm:metzlertheroem}, the system $L_2$ gain from the attack signal $\boldsymbol w(t)$ to the output $\boldsymbol y(t)$ of  \eqref{eqn:attackmain} is given by the largest singular value of $-CA^{-1}B$. With this in mind, we define the game as follows: 

\begin{tcolorbox}
\textbf{Attacker-Detector Game:} The set of attackers $\mathcal{A}$  tries to apply attack signals to some nodes in the network, i.e., determine matrix $B$, to minimize the system $L_2$ gain \eqref{eqn:l2gain}, i.e., provides as small output $\boldsymbol{y}(t)$ as possible, while the detector set $\mathcal{D}$ tries to assign sensors to nodes, i.e., determine matrix $C$, to maximize the $L_2$ gain, i.e., the effect of attacks becomes more apparent in output $\boldsymbol{y}(t)$.  
\end{tcolorbox}

Based on the above definition of the game, the attacker and detector set form a variation of the matrix game. For the case where $f=1$, the well-known matrix game is formed whose payoff is $[A^{-1}]_{ij}$. For the case where $f>1$ the payoff will be the largest singular value of nonnegative matrix $-CA^{-1}B$. In this direction,  we need the following lemma which will be used throughout the paper. 

\begin{lemma}[\cite{vanmeighem}]\label{lem:vanmeigh}
If one element in a nonnegative matrix $M$ is increased, then the largest
eigenvalue (singular value\footnote{The extension to the singular value in this lemma is due to the nonnegativity of matrix $M$.}) is also increased. The increase is strict for irreducible matrices. 
\end{lemma}

In order to further clarification of the game, we present the following remarks. 

\begin{remark}\textbf{(Attackers Prior Knowledge):}
It should be noted that the set of attackers do not have access to matrix $C$, i.e., the set of sensors, and the detectors have not accessed to matrix $B$, i.e., they don't know the attacker set. We will also discuss the case where the attacker set has a prior knowledge about the locations of the detectors and both attacker and detector sets optimize their strategy under the Stackelberg game approach.
We should note that the game analyzed in this paper is a static game, in which the attackers and detectors sets only do a single action. 
\end{remark}


In the following section, we discuss the existence of Nash equilibrium for the attacker-detector game on dynamics \eqref{eqn:attackmain}.


 \section{Existence of Nash Equilibrium for Attacker-Detector Game}
 
  We discuss the  existence pure Nash equilibrium for the attacker-detector game introduced in the previous section.  We start with the following theorem. 
\begin{theorem}\label{thm:noequilibrium}
If matrix $A$ in \eqref{eqn:attackmain} is strictly row and column diagonally dominant, then the attacker-detector game on \eqref{eqn:attackmain} does not have a saddle point equilibrium.
\end{theorem}
\begin{proof}
We should first indicate that a Metzler matrix $A$ which is strictly row and column diagonally dominant has a property that $[A^{-1}]_{ij}< [A^{-1}]_{ii}$ and $[A^{-1}]_{ji}< [A^{-1}]_{ii}$, for all $i,j=1, 2, ...,n$ \cite{Catral}. Based on the definition, a saddle point equilibrium should satisfy
\begin{equation}\label{eqn:sdgjb}
[A^{-1}]_{ij^*}\leq [A^{-1}]_{i^*j^*}\leq [A^{-1}]_{i^*j}
\end{equation}
for all $i=1, 2, ..., n$ and $j=1, 2, ..., n$, where $i^*$ and $j^*$ are the equilibrium strategies for the attacker and detector. Element $ [A^{-1}]_{i^*j^*}$ is either a diagonal element or an off-diagonal element. According to the properties of $A$, if $ [A^{-1}]_{i^*j^*}$ is a diagonal element, then we have $[A^{-1}]_{i^*j^*}> [A^{-1}]_{i^*k}$ for any $k\neq i^*$ and the right inequality of \eqref{eqn:sdgjb} will be violated. Moreover, if it is an off-diagonal element then we have $[A^{-1}]_{i^*j^*} <  [A^{-1}]_{j^*j^*}$ where the left inequality in \eqref{eqn:sdgjb} is violated and this proves the claim. 
\end{proof}
 
 Theorem \ref{thm:noequilibrium} requires that matrix $A$ to be strictly diagonally dominant. This means that systems with non-strict diagonally dominant matrix $A$ (also called quasi-diagonally dominant) may have Nash equilibrium. Examples for cases which are not included in Theorem \ref{thm:noequilibrium} are shown in Table \ref{fig:s4gtdnj}. This table shows that one can not conclude about the existence of NE for the cases where $f>1$ or quasi-diagonally dominant $A$.
 For this in mind, we focus on specific, but important, class of system \ref{eqn:attackmain} and discuss the graph-theoretic interpretations of the existence and the value of the Nash equilibrium.
 

\begin{figure}[t!]
\centering
\includegraphics[scale=.4]{table.pdf}
\caption{Examples for cases which are not included in Theorem \ref{thm:noequilibrium}.  Matrix $A$ in each examples is Metzler and its diagonally dominancy is indicated in the table. }
\label{fig:s4gtdnj}
\end{figure}
 
 
 
 
 
In the following remark we discuss the effect of the existence of multiple leaders, instead of a single leader, on the game payoff.

\begin{remark}\textbf{(Effect of Multiple Leaders):} Based on the proof of Lemma \ref{lem:treehinf}, existence of multiple leaders results in decreasing the value of $[L_g^{-1}]_{ij}$. More formally, we have 
$$[L_g^{-1}]_{ij}\leq \min_{\ell\in \mathcal{S}}|\mathcal{P}_{i\ell} \cap \mathcal{P}_{j\ell}|,$$
where $\mathcal{S}$ is the set of leaders. This makes the payoff value smaller which is not desirable from the detector's perspective. From now, in order to focus on the role of the network structure on the existence of the equilibrium and the game value, we fix $|\mathcal{S}|=1$.
\end{remark}



%%%%%%%%%%Weighted version %%%%%%%%%%%

==> CDC2019 (3)/intro.tex <==



\section{Introduction}

\subsection{Motivation}
The resilience of cyber-physical systems to strategic attacks is one of the primary concerns in the design level and real-time operation of interconnected systems. Examples of such systems include power networks,  water and gas networks, and transportation systems. A subtle difference between faults and attacks is that in the latter, the attacker uses knowledge of vulnerabilities  to maximize its effect and/or minimize its visibility or effort to attack.  The defender thus has to adopt an intelligent strategy to counter the attacker. One approach to modeling interactions between intelligent attackers and defenders is via game theory. 

\subsection{Related Work}

Security and resilience of cyber-physical systems from the game-theoretic standpoint has attracted attention in the past decade; see \cite{zhubasar, Manshaie, Cedricbasar, Amin2013, Aminn, Piranigame } and references therein. The notion of {\it games-in-games} in cyber-physical systems reflects two  interconnected games, one in the cyber layer and the other in the physical layer, for which the payoff of each game affects the result of the other one \cite{Basarz}. Some approaches discussed appropriate game strategies, e.g., Nash or Stackelberg, based on the type of adversarial behavior (active or passive) \cite{Cedricbasar,EPFL}. The evolution of  networked systems are modeled as cooperative games \cite{Mardenshamma} and the resilience of these games to adversarial actions and/or communication failures are investigated \cite{Brown, Shankar}. There is a large literature on the security of first and second order systems \cite{dibaji2017resilient, shames, Hogan}. To date, no approach uses game theory to model the actions of intelligent attackers and defenders in second order  systems.






\subsection{Contributions}
The contributions of this paper are as follows:

\begin{itemize}
 \item We discuss an attacker-defender game on the resilience of two canonical forms of second order systems.  The attacker targets a set of nodes in the network to maximize the system $\mathcal{H}_2$ norm from the attack signals to the output, while the defender  chooses a set of nodes (to install feedback control) in order to minimize this system norm (or mitigate the effect of the attack). 
 
 \item Necessary and Sufficient conditions for the existence of Nash equilibrium (NE) for the game for each of the two second-order dynamics is discussed (Propositions \ref{prop:necsufgame1} and  \ref{prop:none}). For the cases where there is no NE, a Stackelberg game is discussed when the defender acts as the game leader (Theorems \ref{thm:necsuefgame} and \ref{thm:complexx} and Corollary \ref{cor:costfew}). 
 
 \item  For the case of a single attacked node and a single defense node, it is shown that the optimal location of the defense node in the network for each of the second order systems introduces a specific network centrality measure (Remark \ref{rem:ssodjnf}). 
 
 
 \item The extension of the game to the case of multiple attacked and defense nodes is also addressed (Theorems \ref{thm:multistack}, and \ref{thm:complex}).\footnote{ Proofs of all the results of this paper are placed in the Appendix.}
\end{itemize}

It worth noting that for resilient distributed control algorithms proposed in the literature,  a large level of network connectivity is  required to bypass the effects of malicious actions \cite{Hogan, AntonioBicchi}. However, in many real-world applications, e.g., power systems, the underlying topology is designed and can not be changed. From this view, the defense mechanism proposed in this paper has an advantage compared to the previous methods in the sense that it does not rely on the connectivity level of the underlying network.



==> CDC2019 (3)/user_newcommands.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RANDOM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addtolength{\headheight}{14pt}
%\newcommand{\xend}{\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill \quad\hbox{\ensuremath{\lozenge}}} % end environment (e.g. example)
\newcommand{\addcontentslineX}[3]{\phantomsection \addcontentsline{#1}{#2}{#3}} % this command guarantees correct hyperlinks in the pdf to those sections that are not numbered (e.g. acknowledgements, summary, etc.)
\newcommand{\todo}[1] {\textcolor{red}{{#1}}}
\def\str{\color{red}} %STart Red
\def\stb{\color{black}} %STart Black
\newcommand{\publ}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COLOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% cross text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[normalem]{ulem} % either use this (simple) or
%\usepackage{soul}
%\usepackage{cancel}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BIBLIOGRAPHY
% Commands for full citations (NoHyper is used to  solve conflict with hyperref)
% \fullciteInclude includes full citation into bibliography
% \fullciteExclude excludes full citation from bibliography
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\fullcite}[1]{\begin{NoHyper} \bibentry{#1} \end{NoHyper}}
%\DeclareBibliographyCategory{fullcited}
%\newcommand{\mybibexclude}[1]{\addtocategory{fullcited}{#1}}
%\newcommand{\fullciteInclude}[1]{\begin{NoHyper} \fullcite{#1} \end{NoHyper}}
%\newcommand{\fullciteExclude}[1]{\begin{NoHyper} \fullcite{#1}\mybibexclude{#1} \end{NoHyper}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FIGURES
% Commands for including figures/plots in a standard sizing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includegraphicsfig}[1] {\includegraphics[width=80mm,height=60mm,keepaspectratio]{#1}} % Include figure
\newcommand{\includegraphicsplot}[1] {\includegraphics[width=95mm]{#1}} % Include MATLAB plot
%\usepackage{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% MATH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bal}[1] {\ensuremath{\left(\begin{array}{#1}}}
\newcommand{\ear} {\ensuremath{\end{array}\right)}}
\newcommand{\pd}[2] {\ensuremath{\frac{\partial #1}{\partial #2}}}
%\newcommand{\col}[1] {\ensuremath{\left(#1\right)^T}} %column vector in math mode
%\newcommand{\diag}[1] {\ensuremath{\mathrm{diag}\left(#1\right)}} %diagonal matrix in math mode
%\newcommand{\bdiag}[1] {\ensuremath{\mathrm{block.diag}\left(#1\right)}} %diagonal matrix in math mode
\newcommand{\col}[1] {\ensuremath{#1^T}} %column vector in math mode
%\newcommand{\diag}[1] {\ensuremath{\mathrm{diag}(#1)}} %diagonal matrix in math mode
\newcommand{\bdiag}[1] {\ensuremath{\mathrm{block.diag}(#1)}} %diagonal matrix in math mode
\newcommand{\bals}[1] {\ensuremath{\left[\begin{array}{#1}}} % Begin Array Left Square
\newcommand{\ears} {\ensuremath{\end{array} \right] }} % End Array Right Square
%\newcommand{\one}[1] {\ensuremath{\mathds{1}_{#1} }} % Vector of ones
\newcommand{\co} {\ensuremath{\mathrm{co}}} % Convex hull



\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\spa}{span}
\DeclareMathOperator{\sat}{sat}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\inte}{int}
\DeclareMathOperator{\clo}{cl}
\DeclareMathOperator{\rint}{rint}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\atan2}{atan2}
\DeclareMathOperator{\SAT}{SAT}
\DeclareMathOperator{\supp}{supp}
%\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\blcdiag}{blockdiag}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\sinc}{sinc}
%\DeclareMathOperator{\acos}{arccos}


\newcommand{\one} {\ensuremath{\mathds{1} }} % Vector of ones
\newcommand{\T}{\ensuremath{\top}}

\newcommand{\funcRdR}{\ensuremath{{f}}}
\newcommand{\funcRdRd}{\ensuremath{{f}}}

%\DeclareMathOperator{\ones}{{\ensuremath\mathds{1}_n}}

\newcommand{\signf}[1]{\ensuremath{\sign \left( #1 \right)}} % sign function
\DeclareMathOperator*{\bigtimes}{\raisebox{-0.3ex}{\text{\Large$\times$}}}
\newcommand{\inproduct}[1]{\ensuremath{\left\langle #1 \right\rangle}}

\let\leq\leqslant
\let\geq\geqslant
\let\emptyset\varnothing

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

\newcommand{\frakm}{\ensuremath{\mathfrak{m}}} % the lebesgue measure
\newcommand{\frakso}{\ensuremath{\mathfrak{so}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bmat}{\begin{matrix}}
\newcommand{\emat}{\end{matrix}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}
\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\beq*}{\begin{equation*}}
%\newcommand{\eeq*}{\end{equation*}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beni}{\renewcommand{\labelenumi}{\roman{enumi}.}
\renewcommand{\theenumi}{\roman{enumi}}\begin{enumerate}}
\newcommand{\eeni}{\end{enumerate}\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\theenumi}{\arabic{enumi}}}
\newcommand{\bena}{\renewcommand{\labelenumi}{\alpha{enumi}.}
\renewcommand{\theenumi}{\alpha{enumi}}\begin{enumerate}}
\newcommand{\eena}{\end{enumerate}\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\theenumi}{\arabic{enumi}}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SHORTHAND MATH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ones}{\ensuremath{1\!\!1}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\inv}{\ensuremath{^{-1}}}
\newcommand{\pset}[1]{\ensuremath{\{#1\}}}
\newcommand{\nset}[1]{\ensuremath{\{1,2,\ldots,#1\}}}
\newcommand{\setzero}{\ensuremath{\pset{0}}}
\newcommand{\lexleq}{\ensuremath{\preccurlyeq}}
\newcommand{\lexgeq}{\ensuremath{\succcurlyeq}}
\newcommand{\set}[2]{\ensuremath{\{#1\mid #2\}}}
\newcommand{\res}[2]{\ensuremath{#1|_{#2}}}
\newcommand{\abs}[1]{\ensuremath{| #1 |}}
\newcommand{\norm}[1]{\ensuremath{\| #1 \|}}
\newcommand{\inn}[2]{\ensuremath{\langle #1 , #2 \rangle}}
\newcommand{\polar}[1]{\ensuremath{{#1}^\circ}}
\newcommand{\dual}[1]{\ensuremath{{#1}^*}}
\newcommand{\barrier}[1]{\ensuremath{{#1}^{\mathrm{b}}}}
\newcommand{\rec}[1]{\ensuremath{{#1}^{\infty}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SETS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\C}{\ensuremath{\mathbb C}}
\newcommand{\N}{\ensuremath{\mathbb N}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\Lone}{\ensuremath{L_1}}
\newcommand{\Loneloc}{\ensuremath{L_{1,\mathrm{loc}}}}
\newcommand{\Ltwo}{\ensuremath{L_2}}
\newcommand{\Ltwoloc}{\ensuremath{L_{2,\mathrm{loc}}}}
\newcommand{\Linf}{\ensuremath{L_\infty}}
\newcommand{\Linfloc}{\ensuremath{L_{\infty,\mathrm{loc}}}}
\newcommand{\Cinf}{\ensuremath{C^\infty}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  EMPTY CHAPTER PAGES BEFORE EACH CHAPTER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcounter{foochapter} % counter for chapter frontpage
%
%\newcommand{\addchapterfront}{
%\setcounter{foochapter}{\the\value{chapter}}
%\stepcounter{foochapter}
%\cleardoublepage
%\thispagestyle{empty}
%\vspace*{40mm}
%\begin{flushright}
%\fontfamily{ugm}\textrm{\huge Chapter~}
%\color{RoyalRed}\fontfamily{ugm}\fontsize{70}{70}\selectfont\the\value{foochapter} \\
%\vspace{2mm}
%\color{black}\hrule
%\vspace{2mm}
%\includegraphics[height = 20.3mm]{./front/bw_logo_rug}
%%{ \Large \nameref*{chap:\the\value{foochapter}} }
%\end{flushright}
%\renewcommand{\thepage}{[\arabic{page}]}
%\cleardoublepage
%\addtocounter{page}{-2}
%\renewcommand{\thepage}{\arabic{page}}
%}
%
%\newcommand{\addappendixfront}{
%\cleardoublepage
%\thispagestyle{empty}
%\vspace*{40mm}
%\begin{flushright}
%\textbf{\huge Appendix }\\
%\vspace{2mm}
%\hrule
%\end{flushright}
%\renewcommand{\thepage}{[\arabic{page}]}
%\cleardoublepage
%\addtocounter{page}{-2}
%\renewcommand{\thepage}{\arabic{page}}
%}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FONTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\renewcommand{\sfdefault}{mdugm}
%\renewcommand{\sfdefault}{ugm}




%\newboolean{garamond}
%\DeclareOption{garamond}{\setboolean{garamond}{true}}
%
%\ifthenelse{\boolean{garamond}}
%{%
%  \ifpdf
%   \RequirePackage[T1]{fontenc}
%   \RequirePackage[urw-garamond]{mathdesign}
%   \RequirePackage[scaled]{berasans}
%   \RequirePackage{inconsolata} % tt
%   \linespread{1.0609}
%  \fi}%
%{}


==> extra_results.tex <==

\begin{definition}\textbf{(Resistance Distance):}
 The  resistance distance $\mathfrak{R}_{ij}$ between two vertices $v_i$ and $v_j$ in an undirected graph is the equivalent resistance between these two vertices when we treat each edge of the graph as a $1 \Omega$ resistor. \label{def:sldigub}
 \end{definition}

 For the resistance distance $\mathfrak{R}_{i,j}$ and the minimum physical distance between two nodes $\mathfrak{D}_{i,j}$, we have $\mathfrak{R}_{i,j}\leq \mathfrak{D}_{i,j}$, with equality if there exists one path between $v_i$ and $v_j$. Moreover, it can be shown that the resistance distance between $v_{\ell}$ and $v_j$ is the $j$-th diagonal element of $\mathcal{L}_{g{\ell}}^{-1}$, where $v_{\ell}$ is a single grounded vertex \cite{Bapat}. 




\begin{theorem}\label{thm:upperresis}
Consider a connected undirected graph $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ with a set of leaders $\mathfrak{S} \subset \mathcal{V}$.  Let $\mathcal{L}_g$ be the grounded Laplacian matrix induced by $\mathfrak{S}$. Then for the $\mathcal{H}_{\infty}$ norm of \eqref{eqn:partial4} for $\mathcal{B}=\mathbf{e}_i$ and $\mathcal{C}=\mathbf{e}_j^T$ we have
\begin{align}\label{eqn:roofad}
||G||_{\infty} \leq \min\{\min_{\ell \in \mathfrak{S}} \mathfrak{R}_{i,\ell}, \min_{\ell \in \mathfrak{S}}\mathfrak{R}_{j,\ell}\},
\end{align}
with equality when  $i=j$ and $|\mathfrak{S}|=1$.
\end{theorem}
\begin{proof}
The proof is based on the fact that 2-tree $t_{ij,\ell \ell}$ is also a 2-tree $t_{ii,\ell \ell}$, but the inverse is not true. Hence, the cardinality of set of 2-trees $t_{ii,\ell \ell}$ is larger than that of $t_{ij,\ell \ell}$. As a result, based on Lemma \ref{lem:jlsdhav} we conclude that $[\mathcal{L}^
{-1}]_{ij}\leq \min\{[\mathcal{L}^
{-1}]_{ii}, [\mathcal{L}^
{-1}]_{jj}\}$ and based on Definition \ref{def:sldigub} the result is obtained. 

The equality for the case where $i=j$ and there is a  single leader, $\ell$, is clear due to the fact that  $[\mathcal{L}_{g}^{-1}]_{ii}=\mathfrak{R}_{i,\ell}$. however, if $i=j$ and we add more leaders, their effects are considered by diagonal matrix $E=\sum_{k\in \mathcal{V}}\Gamma_k\mathbf{e}_k\mathbf{e}_k^T$, where  $\Gamma_k$ is the number of leaders connected to follower $v_k$. Then, for each matrix $\mathbf{e}_k\mathbf{e}_k^T$ we use Sherman-Morrison formula to get
\begin{align}\label{eqn:vnoswfup}
\Tilde{\mathcal{L}}_{g}^{-1}=\left( \mathcal{L}_{g} + \mathbf{e}_k\mathbf{e}_k^T \right)^{-1}=\mathcal{L}_{g}^{-1}-\frac{\mathcal{L}_{g}^{-1}\mathbf{e}_k\mathbf{e}_k^T\mathcal{L}_{g}^{-1}}{1+\mathbf{e}_k^T\mathcal{L}_{g}^{-1}\mathbf{e}_k}.
\end{align}
Based on the fact that $\mathcal{L}_{g}^{-1}$ is a nonnegative matrix, we conclude from \eqref{eqn:vnoswfup} that the elements of $\tilde{\mathcal{L}}_{g}^{-1}$ will be not larger than those of $\mathcal{L}_{g}^{-1}$, so as its diagonal elements, and this proves the claim. 
\end{proof}

Clearly, when the underlying graph is a tree, based on Theorem \ref{thm:upperresis} we have $||G||_{\infty} \leq \min\{\min_{\ell \in \mathfrak{S}} \mathfrak{D}_{i,\ell}, \min_{\ell \in \mathfrak{S}}\mathfrak{D}_{j,\ell}\}$ with equality if $i=j$ and $|\mathfrak{S}|=1$. The bound mentioned in Theorem \ref{thm:upperresis} are loose in some cases. One of such examples is shown in Fig. \ref{fig:sstdvqwefnj}. In this figure, which is a tree, we have $\mathfrak{R}_{i\ell}=\mathfrak{R}_{j\ell}=3$, while $[\mathcal{L}^
{-1}]_{ij}=1$. 





















\subsection{Mixed Strategy}

For the case of mixed strategy, as stated in Lemmas \ref{lem:blaiug} and \ref{lem:puremix}, upper and lower bounds on the value of the game were proposed. In the context of our case study which is the leader-follower dynamics on trees, we apply these results. Moreover, we compare case of directed trees and undirected trees to examine reducible matrix $L_g^{-1}$ where we have equality $v(L_g^{-1})=\rho(L_g^{-1})$. More formally, we present the following theorem.

\begin{proposition}\label{prop:asjDB}
Let $\mathcal{G}$ be an undirected tree satisfying Assumption 1. Then for the value of mixed game we have $v(L_g^{-1})\geq 1$ and $v(L_g^{-1})> 1$ for complete mixed strategy.
\end{proposition}
\begin{proof}
According to Lemma \ref{lem:puremix} since we have $[L_g^{-1}]_{ij}\geq 1$ for all $i,j=1,2,...n-1$ for undirected trees, the result is proved.
\end{proof}
Based on the above proposition, we present the following important corollary.
\begin{corollary}\label{cor:mixedtreeee}
Let $\mathcal{G}$ be an undirected tree satisfying Assumption 1 and let $\Bar{\mathcal{G}}$ be the directed version of $\mathcal{G}$ with the leader as the source node, i.e., $d_{\rm in}^{\ell}=0$. If $v$ is the mix strategy value for undirected graph and $\Bar{v}$ is the mixed strategy value for directed graph. Then  $v(L_g^{-1})\geq \Bar{v}(L_g^{-1})$.
\end{corollary}
\begin{proof}
According to Proposition \ref{prop:asjDB} we have that $v(L_g^{-1})\geq 1$. However, for directed trees, according to Lemma \ref{lem:blaiug} since $L_g^{-1}$ is reducible we have $\Bar{v}(L_g^{-1})=\rho(L_g^{-1})$. On the other hand since $L_g^{-1}$ is triangular, we have $\rho(L_g^{-1})=\frac{1}{d_{\rm min}}=1$ which proves the claim. 
\end{proof}





 
 \iffalse
 
 
 
 \subsection{Mixed Strategy}
 As, according to Theorem \ref{thm:noequilibrium}, there is no saddle point equilibrium for the pure strategy, we look at the mixed strategy for which the detector and the attacker are choosing a node with a specific probability. More formally, the attacker chooses each node $v_i$ with probability $x_i$ to attack and the detector chooses node $v_i$ with probability ${y}_i$. Clearly $\sum_{i=1}^nx_i=\sum_{i=1}^ny_i=1$. The game is called complete mixed if $x_i,y_i>0$ for all $i=1, 2, ...,n$. For the mixed strategy, the average value of the outcome of the game, corresponding to the strategy pair $\{B,C\}$, will be equal to 
 \begin{equation}
    J(x,y)=\sum_{i=1}^n\sum_{j=1}^nx_i[A^{-1}]_{ij}y_j=\boldsymbol x^TA^{-1}\boldsymbol y,
 \end{equation}
 where $\boldsymbol x=[x_1, x_2, ..., x_n]^T$ and $\boldsymbol y=[y_1, y_2, ..., y_n]^T$ are probability distribution vectors. The attacker tends to minimize and the detector tries to maximize $J(x,y)$  by assigning probability distribution vectors $\boldsymbol x$ and $\boldsymbol y$, respectively. Unlike pure strategy, it is well-known that the mixed strategy always has a saddle point equilibrium, i.e., there are always $\boldsymbol x^*$ and $\boldsymbol y^*$ such that 
 \begin{equation}
\boldsymbol x^*^TA^{-1}\boldsymbol y\leq \boldsymbol x^*^TA^{-1}\boldsymbol y^*\leq \boldsymbol x^TA^{-1} \boldsymbol y^*, \forall \boldsymbol x \in \boldsymbol X, \boldsymbol x \in \boldsymbol Y.
 \end{equation}
 where $\boldsymbol X\triangleq \{\boldsymbol x\in \mathbb{R}^n:\boldsymbol x\geq 0, \sum_{i=1}^nx_i=1\}$, $\boldsymbol Y\triangleq \{\boldsymbol y\in \mathbb{R}^n:\boldsymbol y\geq 0, \sum_{i=1}^ny_i=1\}$.

Using the nonnegativity of $A^{-1}$, we introduce the following two lemmas which give some bounds on the mixed game value and will be used later in Section \ref{sec:netint}.
\begin{lemma}[\cite{Cohen}]\label{lem:blaiug}
For the value of the mixed single attacker-detector game on \eqref{eqn:attackmain} we have $v(A^{-1})\leq \rho(A^{-1})$ with equality if and only if $A^{-1}$ is a reducible matrix, where $\rho$ is the spectral radius of a matrix. 
\end{lemma}

 \begin{lemma}\label{lem:puremix}
 For the value of the mixed single attacker-detector game on \eqref{eqn:attackmain} we have  $v(A^{-1})\geq \max_i\min_j[A^{-1}]_{ij}$ with strict inequality if  the game is completely mixed.
\end{lemma}
\begin{proof}
Based on the definition we have $v(A^{-1})=\max_{\boldsymbol x}\min_{\boldsymbol y}\boldsymbol x^TA^{-1}\boldsymbol y$ for all $\boldsymbol x,\boldsymbol y\geq 0$ where $\mathbf{1}^T\boldsymbol x=\mathbf{1}^T\boldsymbol y=1$. We choose $\boldsymbol x=\textbf{e}_i$ where $i=\arg\max_i\min_j[A^{-1}]_{ij}$. This gives  
\begin{equation}
v(A^{-1})\geq \min_{\boldsymbol y}\textbf{e}_i^TA^{-1}\boldsymbol y= \min_{\boldsymbol y}[A^{-1}]_i\boldsymbol y\geq \max_i\min_j[A^{-1}]_{ij},
\label{eqn:aSEOJgb}
\end{equation} 
where $[A^{-1}]_i$ is the $i-$th row of $A^{-1}$. The right inequality in \eqref{eqn:aSEOJgb} is due to the fact that $\mathbf{1}^T\boldsymbol y=1$ which gives a convex combination of the elements of the $i-$th row of $A^{-1}$ which is not smaller than $\max_i\min_j[A^{-1}]_{ij}$. For the case of complete mixed game, i.e., $\boldsymbol y>0$, we have \eqref{eqn:aSEOJgb} as
\begin{align}
v(A^{-1}) \geq  \min_{\boldsymbol y}[A^{-1}]_i\boldsymbol y>\max_i\min_j[A^{-1}]_{ij}.
\end{align}
\end{proof}
 
In the following section, we will focus on a specific class of dynamics \eqref{eqn:attackmain}, called leader-follower dynamics.
 
 
 
 
 \fi
 
 
 
 
 %%%%%% General Metzler matrices
 
 
 Consider a network of agents $\mathcal{G}=\{\mathcal{V}, \mathcal{E}\}$ where each agent $v_i$ has a scalar and real valued state $x_i(t)$, where $t$ is the time index, and is able to communicate with its neighbors and update its state via the following dynamics 
 \begin{equation}\label{eqn:11}
\dot{x}_i(t)=-a_{ii}x_i(t)+\sum_{j\in \mathcal{N}_i}a_{ij}x_j(t),
 \end{equation}
 where $a_{ij}$s are some positive and constant weights. In addition to \eqref{eqn:11} the updating rule of each agent is prone to an intrusion (or attack). More particularly, there exists a set of attackers $\mathcal{A}$ which inject $f$ attack signals to $f$ nodes in the network. \footnote{The number of attackers in practice is unknown and we can assume $f$ is an upper bound for the number of attacks.}Hence, if the the dynamics of agent $v_i$ is influenced by an attacker, it will be in the following form 
  \begin{equation}
\dot{x}_i(t)=-a_{ii}x_i(t)+\sum_{j\in \mathcal{N}_i}a_{ij}x_j(t)+w_i(t),
 \end{equation}
 where $w_i(t)>0$ represents the attack signal. To detect the effect of attacks, a set of $f$ dedicated sensors (or detectors), denoted by $\mathcal{D}$, are considered, each of which is placed on a specific node, i.e., 
 \begin{equation}
y_i(t)=x_i(t) \quad {\rm if} \quad v_i\in \mathcal{D}.
 \end{equation}
Aggregating the dynamics of each agent into a matrix form results in the following linear time-invariant network dynamical system
 \begin{align}\label{eqn:attackmain}
\dot{\boldsymbol x}(t)&=A\boldsymbol x(t)+ B\boldsymbol w(t),\nonumber\\
\boldsymbol y(t)&=C\boldsymbol x(t),
 \end{align}
 where $\boldsymbol w(t)$ is a vector of exogenous attack signal and we assume that there exists a nonempty time interval $\tau$ such that $\boldsymbol w(t)> \mathbf{0}$, $\forall t\in \tau$. Clearly, matrices $B$ and $C$ are binary matrices such that $B_{n\times f}=[\textbf{e}_1, \textbf{e}_2, ..., \textbf{e}_f]$  and $C_{f\times n}=[\textbf{e}_1^T; \textbf{e}_2^T; ...; \textbf{e}_f^T]$. In words, there is a single 1 in the $i$-th row (column) of matrix $B$ ($C$) if the $i$-th node is under attack (has a measurement). We assume that $||B||_0 >0$, i.e., there exists at least one attack to the system. An example of such systems is shown in Fig.~\ref{fig:sstdnj}. In this example, a $2\times 2$ matrix is chosen by the attacker and the detector from $A^{-1}$ which is shown in bold. 
 
\begin{figure}[t!]
\centering
\includegraphics[scale=.38]{gamedesign.pdf}
\caption{An Example of an attacker-detector game with $f=2$.}
\label{fig:sstdnj}
\end{figure}

 In this paper we assume that matrix $A$ is chosen to be Hurwitz and $-A$ is Metzler, i.e., its off diagonal elements are nonpositive, and row and column diagonally dominant. Based on the fact that $-A$ is Hurwitz, $-A^{-1}$ will be nonnegative elementwise.  The following definition yields Theorem \ref{thm:metzlertheroem} which is required for the rest of the analysis. 
 \begin{definition}\textbf{(Positive Systems)}:
A linear system is called (internally) positive if and only if its state and output are non-negative for every non-negative input and every non-negative initial state.
\end{definition}
\begin{theorem}[\cite{Rantzer}]
A continuous time linear system $(A, B, C)$ is positive if and only if $A$ is a Metzler-matrix and $B$ and  $C$ are non-negative elementwise.  Moreover, for such a positive system with transfer function $G(s)=C(sI-A)^{-1}B$, the system $L_2$ gain, which is equal to $\mathcal{H}_{\infty}$ norm for LTI systems, will be 
\begin{equation} \label{eqn:l2gain}
\sup_{||\boldsymbol w||_2\neq 0} \frac{||\boldsymbol y||_2}{||\boldsymbol w||_2}=\sigma_n(G(0))=\sigma_n(-CA^{-1}B),
\end{equation}
where  $\sigma_{n}$ is the maximum singular value of matrix $G(0)$ and the $L_2$ norm of signal $\boldsymbol u$ is $||\boldsymbol u||_2^2\triangleq \int_0^{\infty}\boldsymbol u^T\boldsymbol u$.
\label{thm:metzlertheroem}
\end{theorem}
 
Based on Theorem \ref{thm:metzlertheroem}, the system $L_2$ gain from the attack signal $\boldsymbol w(t)$ to the output $\boldsymbol y(t)$ of  \eqref{eqn:attackmain} is given by the largest singular value of $-CA^{-1}B$. With this in mind, we define the game as follows: 

\begin{tcolorbox}
\textbf{Attacker-Detector Game:} The set of attackers $\mathcal{A}$  tries to apply attack signals to some nodes in the network, i.e., determine matrix $B$, to minimize the system $L_2$ gain \eqref{eqn:l2gain}, i.e., provides as small output $\boldsymbol{y}(t)$ as possible, while the detector set $\mathcal{D}$ tries to assign sensors to nodes, i.e., determine matrix $C$, to maximize the $L_2$ gain, i.e., the effect of attacks becomes more apparent in output $\boldsymbol{y}(t)$.  
\end{tcolorbox}

Based on the above definition of the game, the attacker and detector set form a variation of the matrix game. For the case where $f=1$, the well-known matrix game is formed whose payoff is $[A^{-1}]_{ij}$. For the case where $f>1$ the payoff will be the largest singular value of nonnegative matrix $-CA^{-1}B$. In this direction,  we need the following lemma which will be used throughout the paper. 

\begin{lemma}[\cite{vanmeighem}]\label{lem:vanmeigh}
If one element in a nonnegative matrix $M$ is increased, then the largest
eigenvalue (singular value\footnote{The extension to the singular value in this lemma is due to the nonnegativity of matrix $M$.}) is also increased. The increase is strict for irreducible matrices. 
\end{lemma}

In order to further clarification of the game, we present the following remarks. 

\begin{remark}\textbf{(Attackers Prior Knowledge):}
It should be noted that the set of attackers do not have access to matrix $C$, i.e., the set of sensors, and the detectors have not accessed to matrix $B$, i.e., they don't know the attacker set. We will also discuss the case where the attacker set has a prior knowledge about the locations of the detectors and both attacker and detector sets optimize their strategy under the Stackelberg game approach.
We should note that the game analyzed in this paper is a static game, in which the attackers and detectors sets only do a single action. 
\end{remark}


In the following section, we discuss the existence of Nash equilibrium for the attacker-detector game on dynamics \eqref{eqn:attackmain}.


 \section{Existence of Nash Equilibrium for Attacker-Detector Game}
 
  We discuss the  existence pure Nash equilibrium for the attacker-detector game introduced in the previous section.  We start with the following theorem. 
\begin{theorem}\label{thm:noequilibrium}
If matrix $A$ in \eqref{eqn:attackmain} is strictly row and column diagonally dominant, then the attacker-detector game on \eqref{eqn:attackmain} does not have a saddle point equilibrium.
\end{theorem}
\begin{proof}
We should first indicate that a Metzler matrix $A$ which is strictly row and column diagonally dominant has a property that $[A^{-1}]_{ij}< [A^{-1}]_{ii}$ and $[A^{-1}]_{ji}< [A^{-1}]_{ii}$, for all $i,j=1, 2, ...,n$ \cite{Catral}. Based on the definition, a saddle point equilibrium should satisfy
\begin{equation}\label{eqn:sdgjb}
[A^{-1}]_{ij^*}\leq [A^{-1}]_{i^*j^*}\leq [A^{-1}]_{i^*j}
\end{equation}
for all $i=1, 2, ..., n$ and $j=1, 2, ..., n$, where $i^*$ and $j^*$ are the equilibrium strategies for the attacker and detector. Element $ [A^{-1}]_{i^*j^*}$ is either a diagonal element or an off-diagonal element. According to the properties of $A$, if $ [A^{-1}]_{i^*j^*}$ is a diagonal element, then we have $[A^{-1}]_{i^*j^*}> [A^{-1}]_{i^*k}$ for any $k\neq i^*$ and the right inequality of \eqref{eqn:sdgjb} will be violated. Moreover, if it is an off-diagonal element then we have $[A^{-1}]_{i^*j^*} <  [A^{-1}]_{j^*j^*}$ where the left inequality in \eqref{eqn:sdgjb} is violated and this proves the claim. 
\end{proof}
 
 Theorem \ref{thm:noequilibrium} requires that matrix $A$ to be strictly diagonally dominant. This means that systems with non-strict diagonally dominant matrix $A$ (also called quasi-diagonally dominant) may have Nash equilibrium. Examples for cases which are not included in Theorem \ref{thm:noequilibrium} are shown in Table \ref{fig:s4gtdnj}. This table shows that one can not conclude about the existence of NE for the cases where $f>1$ or quasi-diagonally dominant $A$.
 For this in mind, we focus on specific, but important, class of system \ref{eqn:attackmain} and discuss the graph-theoretic interpretations of the existence and the value of the Nash equilibrium.
 

\begin{figure}[t!]
\centering
\includegraphics[scale=.4]{table.pdf}
\caption{Examples for cases which are not included in Theorem \ref{thm:noequilibrium}.  Matrix $A$ in each examples is Metzler and its diagonally dominancy is indicated in the table. }
\label{fig:s4gtdnj}
\end{figure}
 
 
 
 
 
In the following remark we discuss the effect of the existence of multiple leaders, instead of a single leader, on the game payoff.

\begin{remark}\textbf{(Effect of Multiple Leaders):} Based on the proof of Lemma \ref{lem:treehinf}, existence of multiple leaders results in decreasing the value of $[L_g^{-1}]_{ij}$. More formally, we have 
$$[L_g^{-1}]_{ij}\leq \min_{\ell\in \mathcal{S}}|\mathcal{P}_{i\ell} \cap \mathcal{P}_{j\ell}|,$$
where $\mathcal{S}$ is the set of leaders. This makes the payoff value smaller which is not desirable from the detector's perspective. From now, in order to focus on the role of the network structure on the existence of the equilibrium and the game value, we fix $|\mathcal{S}|=1$.
\end{remark}



%%%%%%%%%%Weighted version %%%%%%%%%%%
